Formal Aspects of Language Modeling

Large language models have become one of the most commonly deployed NLP inventions. In the past half-decade, their integration into core natural language processing tools has dramatically increased the performance of such tools, and they have entered the public discourse surrounding artificial intelligence. Consequently, it is important for both developers and researchers alike to understand the mathematical foundations of large language models, as well as how to implement them. These notes are the accompaniment to the theoretical portion of the ETH Z\"urich course on large language models, covering what constitutes a language model from a formal, theoretical perspective.

==> chapters/neural-lms/state-space-models.tex <==

\subsection{Kalman Filter}



\subsection{Efficiency of Neural Sequence Modeling}

\subsubsection{Parallelism}

\subsubsection{Computational Complexity}



\subsection{Computational Tricks}

\subsubsection{Parallel Scan}

\subsubsection{Convolution}

\subsubsection{Hierarchy of Memory}


==> chapters/neural-lms/transformers-algorithms.tex <==

\subsection{Algorithmic View}
\Clara{The biggest issue that I see right now (and something hat Ryan will for sure get hung up) is that the section is not self-contained w.r.t. the previous chapters. there's use of a lot of terminology that hasn't been \emph{formally} defined yet (like 'layer' or 'decoder'). While a lot of this terminology might be widely used, we're trying to be very rigorous, and also  to keep things very consistent across chapters. It might not even make sense to use the common terms (except for perhaps pointing out commonly used names when relevant with something like, 'colloquially, these are referred to as...') since we might have already defined something that encompasses the common term. Maybe these things will be defined in the RNN section but they aren't right now. I would coordinate with the RNN authors to make sure their definitions are what you're expecting (and are basing your text off of). Optimally, you could go into the RNN section and write the definitions yourself so that they can work around \emph{your} definitions, rather than you having to come back later and edit things to fall in line with theirs. }
\Clara{I think the most straightforward way to explain the components of the transformer would be to frame it in terms of \cref{eq:softmax-sequence-model}. So something like: a transformer model is one way of parameterizing the distribution $\pLNSM(\eossym_\tstep \mid \eosstr_{<\tstep}) = \projfuncEosalphabetminusFunc{\embedMtx \,\enc(\eosstr_{<\tstep})}_{\eossym_\tstep}$, where the method for building the representation $\enc(\eosstr_{<\tstep})$ consists of... first using a standard embedding function $\emb(\eossym)$ for each $\eossym_t$ to create initial representations, then iteratively transforming these representations via a series of operations whose aim is to encode contextual information from the other tokens in $\str$...  }
The transformer is an encoder-decoder\clara{have these terms been defined?} model primarily based on the self-attention mechanism. In its more general form, it is made up of two halves, an encoder and a decoder, both composed of multiple identical layers\clara{layer hasnt been defined yet} stacked on top of each other. At a high level, given an input string $\mathbf{x} = (\rx_1, \rx_2, \dots ,\rx_{\ell_{\mathbf{x}}})$, the encoder produces a matrix of contextualized input representations $\mZ \in \R^{\ell_{\mathbf{x}} \times d_{out}}$. The decoder then uses $\mZ$, and a second sequence of tokens\clara{the decoder doesnt use a second sequence of tokens, it produces a second sequence of tokens, right?} $\mathbf{\hat{y}} = (\ry_1, \ry_2, \dots ,\ry_{\ell_{\hat{\mathbf{y}}}})$ to generate a new sequence of tokens $\mathbf{y} = (\ry_1, \ry_2, \dots ,\ry_{\ell_{\hat{\mathbf{y}}}})$. An illustration of the entire transformer architecture is shown in \cref{fig:transformer_architecture}. Note that, contrary to RNNs, transformers have a fixed maximum input length $\ell_{max}$. Input sequences whose length exceeds $\ell_{max}$ are either truncated or split into multiple samples, while input sequences of length $< \ell_{max}$ are usually padded with a special padding token $\texttt{[PAD]}$. 

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/transformer-2017-model.png}
    \caption{A graphical representation of the transformer model from the original publication \citep{vaswani2017}}.
    \label{fig:transformer_architecture}
\end{figure}

Each token is an element of the data vocabulary $\sV$\clara{we use $\alphabet$} and is assigned to a unique index in the $[0, |\sV|-1]$ range called \defn{token ID}\clara{this is already explained in \cref{example:one-hot-encoding}. Would use notation from there}. The \defn{vocabulary} is a finite set of cardinality $|\sV|$ that can be composed of characters, words, or subwords. Defining $\sV$ at the character level, e.g. by using all letters of the English language and punctuation, would yield a small vocabulary but extremely long sequences. On the other hand, a vocabulary composed of all possible words of the English language yields shorter sequence lengths at the expense of very large vocabulary sizes $|\sV|$ and the inability to deal with words encountered during inference but not present in the training data. Subwords, segments making up complete words, offer a favorable trade-off between vocabulary size and sequence length, making them the most commonly used method for building vocabularies in current language models. There are multiple ways to obtain a set of sub-words from a corpus: the process by which a textual string is split into a sequence of vocabulary elements is called \defn{tokenization}\index{tokenization} and is discussed in more detail later in \cref{sec:tokenization}. 

\subsubsection{Input embeddings}\clara{this section needs to be framed in terms of \cref{sec:representation-based-modeling}. I don't this you need to give definitions/explanations for $\ve_t$}
At the beginning of the encoding process, input tokens $\rx_{\ell}$ are transformed into input embeddings $\ve \in \R^{d_e}$. Input embeddings are obtained as the sum of a token embedding  $\ve_t \in \R^{d_e}$ and a positional embedding $\ve_p \in \R^{d_e}$. 
\begin{equation}\label{eq:transformer_input_embeddings}
  \ve = \ve_t + \ve_p   
\end{equation}

Token embeddings are used to represent each vocabulary element as a vector and obtained following \cref{alg:transformer_token_embeddings}. In words, token embeddings are the rows of the learnable token embedding matrix $\mW_e$. Positional embeddings represent the position of a token in the input sequence as a vector. They are necessary to allow the transformer to obtain information on how the input tokens are ordered. If they weren't present, the transformer would be permutation invariant in its inputs\clara{its not yet clear why this is true, which makes me think that this section should perhaps be later}, and would therefore have no way to use the word ordering information, a fundamental property of language. Similarly to token embeddings, as shown in \cref{alg:transformer_positional_embeddings}, positional embeddings are the rows of the positional embedding matrix $\mW_p$. Positional embeddings can be learned or fixed: the original transformer makes use of hard-coded sinusoidal positional embeddings computed using the following formula: 

\begin{align}
& \ve_p = 
\begin{cases}
     \mW_p[l, 2i] = \sin{\left(\frac{l}{\ell_{max}^{2i /d_e}} \right)} \\ 
     \mW_p[l, 2i+1] = \cos{\left(\frac{l}{\ell_{max}^{2i /d_e}} \right)} \\ 
\end{cases} \\
& \text{for } 0 \leq i < d_e / 2 \text{ and } 0 \leq l < \ell_{max} \nonumber
\end{align}


\begin{algorithm}
\textbf{Input:} $\rv \in [0, |\sV|-1]$, a token ID \\
\textbf{Output:} $\ve_t \in \R^{d_e}$ \\
\textbf{Parameters:} $\mW_e \in \R^{|\sV| \times d_e}$, the token embedding matrix 
\begin{algorithmic}[1]
\caption{Token embeddings}\label{alg:transformer_token_embeddings}
    \State \Return $\ve_t = \mW_e[\rv, :]$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\textbf{Input:} $\ell \in [0, \ell_{max}-1]$, token position in the input sequence \\
\textbf{Output:} $\ve_p \in \R^{d_e}$ \\
\textbf{Hyperparameters:} $\mW_p \in \R^{\ell_{max} \times d_e}$, the positional embedding matrix
\begin{algorithmic}[1]\caption{Positional embeddings}\label{alg:transformer_positional_embeddings}
    \State \Return $\ve_p = \mW_p[\ell, :]$
\end{algorithmic}
\end{algorithm}

\subsubsection{The transformer encoder}\Clara{tbh, I'm not sure the encoder component of the transformer model even needs to be discussed since we would focus on decoder only models, right? I suppose things like T5 are encoder-decoder so perhaps the encoder output could be framed as something additional to condition our representation function on when building the representation of the context $\str$, but not sure how much detail is needed. The important part that needs to come through here (but doesnt right now) is that we're framing everything in terms of learning a representation function that can tell us how similar/compatible a word is with its context.  }
The encoder processes the input embeddings through two sublayers: a self-attention sublayer and a feed-forward sublayer. The self-attention sublayer is arguably the most crucial component of the transformer, as it allows the encoder to incorporate contextual information, i.e. information following or preceding each token. To describe how self-attention is calculated with a simple example, we examine its computation when provided with a short input sequence ($\ell_{\mathbf{x}} = 3$) of three tokens: \emph{"Transformers are awesome"}\footnote{Here we assume that all words correspond to a single token in $\sV$. Notice that this might not always be the case when employing subword tokenization.}. We use only the first token as the query. The entire process is shown in ~\cref{fig:transformer_single_query_attention}. At first, the three tokens are mapped to their respective token ID, and, using~\cref{eq:transformer_input_embeddings} to their input embedding. We compute key and value vectors for all tokens, but only query $\vq_1 \in \R^{d_{attn}}$ for the first input embedding $\ve_1 \in \R^{d_{e}}$. We then compute the inner product between $\vq_1$ and each keys, interpreting the inner product score $\rs_{\ell} = \vq\vk_{\ell}^{\top}$ between the query and a contextual key as the importance that $\ve_{\ell}$ has for $\ve$. By repeating this procedure for all keys, we obtain an array of importance scores that we then scale down by a constant value $(\sqrt{d_{attn}})$  for gradient stability, and normalize with the $\operatorname{softmax}$ function. The normalized scores $\alpha_{\ell}$ are known as \defn{attention probabilities}\index{attention!probabilities}. Finally, the output of attention for a single query $\vq_1$ is the weighted average of all the value vectors using the attention probabilities as weights. This particular variant of attention is named \defn{Scaled Dot-Product Attention}\index{attention!scaled}\index{attention!dot-product} and laid out more formally in \cref{alg:transformer_single_query_attention}.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/transformer_single_query_attention.png}
    \caption{Graphical representation of \cref{alg:transformer_single_query_attention} adapted from the \href{https://jalammar.github.io/illustrated-transformer/}{Illustrated Transformer}. Token IDs and attention scores $\rs$ are arbitrary.}
    \label{fig:transformer_single_query_attention}
\end{figure}

\begin{algorithm}
  \textbf{Input:}{
    \begin{tabular}[t]{ll}
      $\ve \in \R^{d_{e}}$& embedding of the current token \\
      $\ve_{\ell} \in \R^{d_{e}}$& $\forall\ \ell: 0 \leq \ell < \ell_{max}$ contextual token embeddings  \\
    \end{tabular}
  } \\
\textbf{Output:}{
    \begin{tabular}[t]{ll}
        $\tilde{\vv} \in \R^{d_{o}}$& contextualized embedding of $\ve$
    \end{tabular}} \\
\textbf{Parameters:}
    \begin{tabular}[t]{ll}
        $\mW_q, \mW_k \in \R^{d_{attn} \times d_{e}}$ & weight matrices for queries and keys\\
        $\vb_q, \vb_k \in \R^{d_{attn}}$ & bias vectors for queries and keys\\
        $\mW_v \in \R^{d_{o} \times d_{e}}$ & weight matrix for values \\
        $\vb_v \in \R^{d_{o}}$ & bias vector for values \\
    \end{tabular}

\begin{algorithmic}[1]
\caption{Single-query Scaled Dot-Product Attention}\label{alg:transformer_single_query_attention}
    \State $\vq \gets \re\mW_q^{\top} + \vb_q$
    \State $\forall \ell: \vk_{\ell} \gets \ve\mW_k^{\top} +  \vb_k$
    \State $\forall \ell: \vv_{\ell} \gets \ve\mW_v^{\top} +  \vb_v$
    \State $\forall \ell: \alpha_{\ell} \gets \frac{\exp{(\vq\vk_t^{\top}/\sqrt{d_{attn}})}}{\sum_u \exp{(\vq\vk_u^{\top}/\sqrt{d_{attn}})}}$ \Comment{Attention probability between $\ve$ and $\ve_{\ell}$}
    \State \Return $\tilde{\vv} = \sum_{\ell=1}^{\ell_{max}} \alpha_{\ell} \vv_{\ell}$
\end{algorithmic}
\end{algorithm}

In practice, for faster processing, attention is computed using multiple queries in matrix form. In this form, the computation of attention follows \cref{alg:transformer_attention}. Depending on how we define $\mZ$ different attention variants are possible: If $\mX = \mZ$, the input and contextual sequences are equivalent and \cref{alg:transformer_attention} is named \defn{self-attention}\index{attention!self}. If $\mX \neq \mZ$, we call it \defn{cross-attention}\index{attention!cross} instead, as attention is computed across two different sequences. Attention also involves the use of a masking matrix $\mM$: depending on the definition of $\mM$, attention can be \defn{masked} (or unidirectional) or \defn{unmasked}\index{attention!masked}\index{attention!unmasked} (or bidirectional). In unmasked attention, the masking matrix $\mM$ is a matrix of ones, and it does not change the content of the score matrix $\mS$. This allows attention to be computed using contextual information positioned both before and after the current token. On the other hand, in masked attention $\mM$ is a lower triangular matrix, zeroing out all tokens preceding the current token in the sequence.

\begin{equation}
\mM[\ell_x, \ell_z] = 
\begin{cases}
    1 \text{ for unmasked attention} \\
    \ell_x \leq \ell_z \text{ for masked attention}
\end{cases}
\end{equation}

\begin{algorithm}
\begin{tabular}{p{0.15\textwidth}p{0.75\textwidth}}
\textbf{Input:} & $\mX, \mZ \in \R^{\ell_{max} \times d_{in}}$, matrix representations of the input and context sequences. \\
\textbf{Output:} & $\tilde{\mV} \in \R^{\ell_{max} \times d_{o}}$, representation of tokens in $\mX$ with contextual information from $\mZ$. \\
\end{tabular} \\
\begin{tabular}{p{0.2\textwidth}p{0.7\textwidth}}
\textbf{Parameters:} & $\headqkvparams$ consisting of: \\
&\quad $\mW_q \in \R^{d_{attn} \times d_{in}}, \vb_q \in \R^{d_{attn}}$, \\
&\quad $\mW_k \in \R^{d_{attn} \times d_{in}}, \vb_k \in \R^{d_{attn}}$, \\
&\quad $\mW_v \in \R^{d_{o} \times d_{in}}, \vb_v \in \R^{d_{o}}$ \\
& weight matrices and bias vectors for queries, keys, and values, respectively. \\
\end{tabular} \\
\begin{tabular}{p{0.25\textwidth}p{0.65\textwidth}}
\textbf{Hyperparameters:} & $\mM \in \R^{\ell_{max} \times \ell_{max}}$, masking matrix. \\
\end{tabular} 
\begin{algorithmic}[1]
    \State $\mQ \gets \mX\mW_q^{\top} + \mathbf{1}^{\top} \vb_q$
    \State $\mK \gets \mZ\mW_k^{\top} + \mathbf{1}^{\top} \vb_k$
    \State $\mV \gets \mZ\mW_v^{\top} + \mathbf{1}^{\top} \vb_v$
    \State $\mS \gets \mQ\mK^{\top}$ \label{line:transformers_score_matrix}
    \State $\forall \ell_x, \ell_z: \text{if } \sim\mM[\ell_x, \ell_z], \text{ then } \mS[\ell_x, \ell_z] \gets -\infty$
    \State \Return $\tilde{\mV} = \softmaxfunc{\frac{S}{\sqrt{d_{attn}}}}{}\mV$
\end{algorithmic}
\caption{$\texttt{Attention}(\mX, \mZ, \headqkvparams, \mM)$}\label{alg:transformer_attention}
\end{algorithm}

Until now, we computed attention using a single set of queries, keys and values. Transformers repeat this process in parallel across multiple \emph{heads}\clara{give formal definintion of a head in a definition environment}, through a variant of attention known as \defn{Multi-Head Attention}. In Multi-Head Attention, different weights matrices and bias\clara{in general, you can omit the bias as an explicit part of the parameters and just have it implicitly encoded in W} vectors are used to create multiple query, key, and value matrices. Attention is them computed in parallel for each of these query, key, and value versions. The output matrices are then concatenated and projected a final time. Multi-Head Attention is shown in \cref{alg:transformer_multihead_attention}.

\begin{algorithm}
\begin{tabular}{p{0.15\textwidth}p{0.75\textwidth}}
\textbf{Input:} & $\mX \in \R^{\ell_{max} \times d_{in}}, \mZ \in \R^{\ell_{max} \times d_{in}}$ matrix representations of the input and context sequences. \\
\textbf{Output:} & $\tilde{\mV} \in \R^{\ell_{max} \times d_{out}}$ representation of tokens in $\mX$ with contextual information from $\mZ$. \\
\end{tabular}
\begin{tabular}{p{0.2\textwidth}p{0.7\textwidth}}
\textbf{Parameters:} & $\multiheadparams$ containing: \\
    & For $\rh \in [0, H-1]$, $\headqkvparams^{\rh}$: \\
    &\quad $\mW_q^h \in \R^{d_{attn} \times d_{in}}, \vb_q^h \in \R^{d_{attn}}$,\\
    &\quad $\mW_k^h \in \R^{d_{attn} \times d_{in}}, \vb_k^h \in \R^{d_{attn}}$, \\
    &\quad $\mW_v^h \in \R^{d_{o} \times d_{in}}, \vb_v^h \in \R^{d_{o}}$, \\
    &weight matrices and bias vectors for queries, keys, and values, respectively, for each head. \\
    & $\mW_o \in \R^{d_{out} \times H d_o}$, $\vb_o \in \R^{d_{out}}$ weight matrix and bias vector for the final projection. \\
\end{tabular}
\begin{tabular}{p{0.25\textwidth}p{0.65\textwidth}}
\textbf{Hyperparameters:} &$H$, number of attention heads, \\
    &$\mM \in \R^{\ell_{max} \times \ell_{max}}$, masking matrix. \\
\end{tabular}
\begin{algorithmic}[1]
    \For{$\rh \in [0, H-1]$}
        $\mY^h \gets \texttt{Attention}(\mX, \mZ, \headqkvparams, \mM)$
    \EndFor
    \State $\mY \gets [\mY^0; \mY^1; \dots; \mY^{H-1}]$
    \State \Return $\tilde{\mV} = \mY\mW_o^{\top} + \mathbf{1}^{\top}\vb_o$
\end{algorithmic}
\caption{$\texttt{MHAttention}(\mX, \mW, \multiheadparams, \mM)$}\label{alg:transformer_multihead_attention}
\end{algorithm}

The main advantage of Multi-Head Attention over its single head variant is that it enhances the model's ability to encode complex patterns, as each head can learn to attend to different aspects of the input sequence.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/transformer_attention.png}
    \caption{(left) Graphical representation of \cref{alg:transformer_single_query_attention}. (right) Graphical representation of \cref{alg:transformer_attention} from~\cite{vaswani2017}.}
    \label{fig:transformer_architecture}
\end{figure}


We now turn our attention to the second sublayer of the transformer encoder: the feed-forward sublayer. This sublayer consists of only two linear projections that are intertwined by an activation function, usually a $\texttt{ReLU}$ or one of its variants. The feed-forward sublayer is specified in \cref{alg:transformer_ffn}.

\begin{algorithm}
\begin{tabular}{p{0.15\textwidth}p{0.75\textwidth}}
\textbf{Input:} & $\tilde{\mV} \in \R^{\ell_{max} \times d_{out}}$ output of an attention layer\\ 
\end{tabular}
\begin{tabular}{p{0.2\textwidth}p{0.7\textwidth}}
\textbf{Parameters:} & $\ffnparams$ consisting of: \\
&\quad $\mW_{mlp1} \in \R^{d_{mlp} \times d_{out}}, \vb_{mlp1} \in \R^{d_{mlp}}$, first linear projection parameters \\
&\quad $\mW_{mlp2} \in \R^{d_{out} \times d_{mlp}}, \vb_{mlp2} \in \R^{d_{out}}$, second linear projection parameters 
\end{tabular}
\begin{tabular}{p{0.25\textwidth}p{0.65\textwidth}}
\textbf{Hyperparameters:} & $\actfn{\cdot}$, activation function \\
\end{tabular}
\begin{algorithmic}[1]
    \State \Return $\actfn{\tilde{\mV}\mW_{mlp1}^{\top} + \mathbf{1}^{\top}\vb_{mlp1}}\mW_{mlp2}^{\top} + \mathbf{1}^{\top}\vb_{mlp2}$
\end{algorithmic}
\caption{$\texttt{FFN}(\tilde{\mV}, \ffnparams, \actfn{\cdot})$}\label{alg:transformer_ffn}
\end{algorithm}

Only one piece of the transformer encoder is missing before we can outline the whole picture: \defn{layer normalization}\index{layer normalization}. Layer normalization~\cite{Lei2016layernorm} is an activation normalization method that is widely adopted in NLP. It normalizes its input vectors independently across the feature dimension, leading to robustness to variations in the scale and distribution of the activations and more stability during training. Layer normalization is shown in \cref{alg:transformer_layernorm}.

\begin{algorithm}
\begin{tabular}{p{0.15\textwidth}p{0.75\textwidth}}
\textbf{Input:} & $\ve \in \R^{d_e}$, neural network activations.\\ 
\textbf{Output:} & $\hat{\ve} \in \R^{d_e}$, normalized activations.\\ 
\end{tabular}
\begin{tabular}{p{0.2\textwidth}p{0.7\textwidth}}
\textbf{Parameters:} & $\boldsymbol{\gamma}, \boldsymbol{\beta} \in \R^{d_e}$, element-wise scale and offset vectors \\
\end{tabular}
\begin{algorithmic}[1]
    \State $\vm \gets \sum_{i=1}^{d_e} \ve[i]/d_e$
    \State $\rv \gets \sum_{i=1}^{d_e}(\ve[i] - \vm)^2/d_e$
    \State \Return $\hat{\ve} \gets \frac{\ve - \vm}{\sqrt{\rv}} \odot \boldsymbol{\gamma} + \boldsymbol{\beta}$
\end{algorithmic}
\caption{$\texttt{LayerNorm}(\ve,\boldsymbol{\gamma},\boldsymbol{\beta} )$}\label{alg:transformer_layernorm}
\end{algorithm}

Using all the algorithms encountered so far, we can finally describe the complete workings of a transformer Encoding. Formally, the encoder is detailed in \cref{alg:transformer_encoder}, graphically, this corresponds to the left half of \cref{fig:transformer_architecture}. At first, the input sequence is encoded by computing an input embedding for each input token ID. The input embeddings are then concatenated into an input matrix $\mX$, which is passed through identical $L_{enc}$ encoder blocks. As shown in lines~\ref{line:transformer_residual_connection1} and~\ref{line:transformer_residual_connection2} of \cref{alg:transformer_encoder}, both halves of each encoder block are followed by a \defn{residual connection}, before being fed to a $\texttt{LayerNorm}$ layer. A residual connection, also known as a skip connection, is a technique used in the transformer model that operates around a sublayer, adding its inputs back into its outputs as follows: 
\begin{equation}
    \mX = \texttt{Sublayer}(\mX) + \mX
\end{equation}
Residual connections, first introduced in~\cite{He2016Residual}, provide gradients with a more direct route that avoids passing through each sublayer when flowing backward though the entire network during backpropagation. This helps mitigating the vanishing gradient problem.

The encoder finally outputs $\mZ$: the output of its last block.

\begin{algorithm}
\begin{tabular}{p{0.15\textwidth}p{0.75\textwidth}}
\textbf{Input:} & $\mathbf{x}$, sequence of token IDs of length $\ell_{\mathbf{x}} \leq \ell_{max}$ \\ 
\textbf{Output:} & $\mZ \in \R^{\ell_{\mathbf{x}} \times d_{out}}$, contextualized representation of the input sequence \\ 
\end{tabular}
\begin{tabular}{p{0.2\textwidth}p{0.7\textwidth}}
\textbf{Parameters:} & $\boldsymbol{\theta}_{enc}$ consisting of the following: \\
& $\mW_e \in \R^{d_e \times |\sV|}, \mW_p \in \R^{d_e \times \ell_{max}}$, token and positional embedding matrices. \\ 
& For $\rl \in [0, L_{enc}-1]:$ \\
& \quad $\multiheadparams_{\rl}$, $\rl$-th Multi-Head Attention parameters. \\
& \quad $\ffnparams_{\rl}$, parameters for the $\rl$-th FNN sublayer. \\
& \quad $\boldsymbol{\gamma}_{\rl}^1, \boldsymbol{\beta}_{\rl}^1, \boldsymbol{\gamma}_{\rl}^2, \boldsymbol{\beta}_{\rl}^2 \in \R^{d_e}$, LayerNorm parameters. \\
\end{tabular}
\begin{algorithmic}[1]
    \For{$\ell \in [0, \ell_{\mathbf{x}}]$} \Comment{Encoding input sequence}
        \State $\ve_{\ell} \gets \mW_e[:, \mathbf{x}[\ell]] + \mW_p[:, \ell]$
    \EndFor
    \State $\mX \gets [\ve_1; \ve_2; \dots \ve_{\ell_{\mathbf{x}}}]$
    \For{$\rl \in [0, L_{enc}-1]$} \Comment{Cycling over $L_{enc}$ encoder blocks}
        \State $\mX \gets \mX + \texttt{MHAttention}(\mX, \mX, \multiheadparams, \mM \equiv 1)$\Comment{Bidirectional self-attention} \label{line:transformer_residual_connection1}
        \For{$\ell \in [0, \ell_{\mathbf{x}}-1]$} $\mX[\ell, :] \gets \texttt{LayerNorm}(\mX[\ell, :],\boldsymbol{\gamma}_{\rl}^1, \boldsymbol{\beta}_{\rl}^1)$ 
        \EndFor
        \State $\mX \gets \mX + \texttt{FFN}(\mX, \ffnparams_{\rl}, \texttt{ReLU})$  \label{line:transformer_residual_connection2}
        \For{$\ell \in [0, \ell_{\mathbf{x}}-1]$} $\mX[\ell, :] \gets \texttt{LayerNorm}(\mX[\ell, :],\boldsymbol{\gamma}_{\rl}^2, \boldsymbol{\beta}_{\rl}^2)$
        \EndFor
    \EndFor
    \State \Return $\mZ \gets \mX$
\end{algorithmic}
\caption{$\texttt{TransformerEncoder}(\boldsymbol{\theta}_{enc}, \mathbf{x})$}\label{alg:transformer_encoder}
\end{algorithm}

\subsubsection{The transformer decoder}

As shown in \cref{fig:transformer_architecture}, the transformer Decoder is composed of identical decoder blocks placed one after the other. Every block is composed of three sublayers, each immediately followed by a residual connection and a $\texttt{LayerNorm}$ layer. The first sublayer is a \emph{masked} multi-head self-attention layer: it has the same structure as the multi-head self-attention sublayer of the encoder, but it uses a unidirectional masking matrix $\mM [\ell, \ell^{'}] = [\ell \leq \ell^{'}]$ that masks out all future tokens and preserves the autoregressive property. The second sublayer is a multi-head \emph{cross}-attention layer: it uses the outputs $\mZ$ of the encoder as keys and values, while the decoded sequence is used as the query. The last layer is a $\texttt{FNN}$ layer equivalent to the one in the encoder. The output of the last decoder block is passed through a final linear layer encoded by the $\mW_u$ matrix and then through a $softmax(\cdot)$ layer. This final operation yields an output matrix $\mP$ whose rows form a normalized probability distribution over the vocabulary. It is worth noting that, in most cases, the \defn{unembedding matrix} $\mW_u$ is fixed to being equivalent to the transpose of the token embedding matrix: $\mW_u^{\top} := \mW_e$.

As we have already defined most components of the transformer Decoder in the previous subsection, we outline its structure in \cref{alg:transformer_decoder}.

\begin{algorithm}
\begin{tabular}{p{0.15\textwidth}p{0.75\textwidth}}
\textbf{Input:} & $\hat{\mathbf{y}}$, sequence of token IDs of length $\ell_{\hat{\mathbf{y}}} \leq \ell_{max}$. \\ 
& $\mZ$, transformer encoder output. \\
\textbf{Output:} & $\mP \in (0, 1)^{\ell_{\hat{\mathbf{y}}} \times |\sV|}$, probability distributions over $\sV$.
\end{tabular}
\begin{tabular}{p{0.18\textwidth}p{0.75\textwidth}}
\textbf{Parameters:} & $\boldsymbol{\theta}_{dec}$ consisting of the following: \\
& $\mW_e \in \R^{d_e \times |\sV|}, \mW_p \in \R^{d_e \times \ell_{max}}$, token and positional embedding matrices. \\ 
& $\mW_u \in \R^{d_e \times |\sV|}$, final projection matrix. \\
& For $\rl \in [0, L_{dec}-1]:$ \\
& \quad $\multiheadparams_{\rl 1}$, $\rl$-th Multi-Head \emph{masked} Attention parameters. \\
& \quad $\multiheadparams_{\rl 2}$, $\rl$-th Multi-Head \emph{cross} Attention parameters. \\
& \quad $\ffnparams_{\rl}$, parameters for the $\rl$-th FNN sublayer. \\
& \quad $\boldsymbol{\gamma}_{\rl}^3, \boldsymbol{\beta}_{\rl}^3, \boldsymbol{\gamma}_{\rl}^4, \boldsymbol{\beta}_{\rl}^4, \boldsymbol{\gamma}_{\rl}^5, \boldsymbol{\beta}_{\rl}^5 \in \R^{d_e}$, LayerNorm parameters. \\
\end{tabular}

\begin{algorithmic}[1]
    \For{$\ell \in [0, \ell_{\hat{\mathbf{y}}}]$} \Comment{Encoding input sequence}
        \State $\ve_{\ell} \gets \mW_e[:, \hat{\mathbf{y}}[\ell]] + \mW_p[:, \ell]$
    \EndFor
    \State $\mY \gets [\ve_1; \ve_2; \dots \ve_{\ell_{\hat{\mathbf{y}}}}]$
    \For{$\rl \in [0, L_{dec}-1]$} \Comment{Cycling over $L_{dec}$ Decoder blocks}
        \State $\mY \gets \mY + \texttt{MHAttention}(\mY, \mY, \multiheadparams_{\rl 1}, \mM[\ell, \ell^{'}] \equiv [\ell \leq \ell^{'}])$ \Comment{Masked self-attention}
        \For{$\ell \in [0, \ell_{\hat{\mathbf{y}}}-1]$} $\mY[\ell, :] \gets \texttt{LayerNorm}(\mY[\ell, :],\boldsymbol{\gamma}_{\rl}^3, \boldsymbol{\beta}_{\rl}^3)$ 
        \EndFor
        \State $\mY \gets \mY + \texttt{MHAttention}(\mY, \mZ, \multiheadparams_{\rl 2}, \mM[\ell, \ell^{'}] \equiv 1)$ \Comment{Cross-attention}
        \For{$\ell \in [0, \ell_{\hat{\mathbf{y}}}-1]$} $\mY[\ell, :] \gets \texttt{LayerNorm}(\mY[\ell, :],\boldsymbol{\gamma}_{\rl}^4, \boldsymbol{\beta}_{\rl}^4)$ 
        \EndFor
        \State $\mY \gets \mY + \texttt{FFN}(\mY, \ffnparams_{\rl}, \texttt{ReLU})$
        \For{$\ell \in [0, \ell_{\hat{\mathbf{y}}}-1]$} $\mY[\ell, :] \gets \texttt{LayerNorm}(\mY[\ell, :],\boldsymbol{\gamma}_{\rl}^5, \boldsymbol{\beta}_{\rl}^5)$
        \EndFor
    \EndFor
    \State \Return $\mP \gets \operatorname{softmax}(\mY \mW_{u}^{\top})$
\end{algorithmic}
\caption{$\texttt{transformerDecoder}(\boldsymbol{\theta}_{dec}, \hat{\mathbf{y}}, \mZ)$}\label{alg:transformer_decoder}
\end{algorithm}

The original transformer from~\cite{vaswani2017} can then be easily outlined in only two lines of pseudocode (\cref{alg:transformer_encoder_decoder}).

\begin{algorithm}
\begin{tabular}{p{0.15\textwidth}p{0.75\textwidth}}
\textbf{Inputs:} & $\mathbf{x}$, sequence of token IDs of length $\ell_{\mathbf{x}} \leq \ell_{max}$ \\ 
& $\hat{\mathbf{y}}$, sequence of token IDs of length $\ell_{\hat{\mathbf{y}}} \leq \ell_{max}$\\
\textbf{Output:} & $\mP \in (0, 1)^{\ell_{\hat{\mathbf{y}}} \times |\sV|}$, probability distributions over $\sV$.
\end{tabular}
\begin{tabular}{p{0.18\textwidth}p{0.75\textwidth}}
\textbf{Parameters:} & $\boldsymbol{\theta}_{T} = \{\boldsymbol{\theta}_{enc}, \boldsymbol{\theta}_{dec} \}$ \\
\end{tabular}

\begin{algorithmic}[1]
    \State $\mZ \gets \texttt{transformerEncoder}(\boldsymbol{\theta}_{enc}, \mathbf{x})$
    \State \Return $\mP \gets \texttt{transformerDecoder}(\boldsymbol{\theta}_{dec}, \mathbf{y}, \mZ)$
\end{algorithmic}
\caption{$\texttt{transformer}(\boldsymbol{\theta}_{dec}, \boldsymbol{\theta}_{enc}, \mathbf{x}, \hat{\mathbf{y}})$}\label{alg:transformer_encoder_decoder}
\end{algorithm}

\subsubsection{Basic transformer variants}

Starting from the full transformer architecture, two variants can be built: an encoder-only transformer and a decoder-only transformer. Encoder-only transformers are used for classification-derived NLP tasks such as sentiment analysis, semantic equivalence, and natural language inference. 

BERT (Bidirectional Encoder Representations from Transformers)~\cite{devlin-etal-2019-bert} is perhaps the most well-known encoder-only transformer and it consists of an transformer encoder with a few modifications. The most important difference between BERT and a transformer encoder is the presence of an additional classification layer after the last transformer encoder block. This classification layer is a linear layer parametrized by parameters $\mW_{cls} \in \R^{C \times d_e}$ and $\vb_{cls} \in \R^{C}$, where $C$ is the task-dependent number of classification classes. A special classification token $\texttt{[CLS]}$\clara{would come up with a new variable that's $\alphabet \cup \texttt{[CLS]}$} is added as the first token of the input sequence, then its contextualized representation $\vz = \mZ[0, :]$\clara{would just index this with \texttt{[CLS]} instead of 0 since the 0 is kind of an arbitrary choice} is passed through the classification layer and a softmax, obtaining a probability distribution $p_c$ over $C$ classes as follows:

\begin{equation}
    p_c = \softmax(\mZ[0, :]\mW_{cls}^{\top} + \vb_{cls}) \in \R^{C}
\end{equation}

For tasks in which classifying the entire sequence is necessary, we can pass the entire encoded representation $\mZ$ through the classification layer, yielding a probability distribution over classes for each input token. BERT also uses $\texttt{GELU}$ as its activation function $\actfn{\cdot}$ instead of $\texttt{ReLU}$, as it was empirically found to increase performance and decrease convergence time. 

GPT (Generative Pretrained Transformer)~\cite{Radford2019GPT} is widely recognized as the most popular decoder-only transformer. Its autoregressive nature makes it particularly appropriate for natural language generation tasks. While subsequent improvements have been made over the years, the original implementation of GPT was practically identical to a single transformer decoder. The most notable architectural differences include the use of the $\texttt{GELU}$ activation function and the removal of the cross-attention sublayer in the decoder blocks. This last change was needed since there is no encoder to produce a $\mZ$ in GPT.



==> chapters/neural-lms/vanishing-gradient.tex <==

\subsection{The Vanishing and Exploding Gradient Problem} \label{sec:vanishing-exploding-gradient}
Let us use the following examples to motivate this subsection.
\begin{example}{Long-term dependency in natural language}{long-term-dependency-nl}
    Considering one of the sentences from \cref{ex:human-language-nonregular}.

    \begin{center}
        \textexample{The cat the dog the mouse the rat frightened startled barked at likes to cuddle.}
    \end{center}

    Questions: Who likes to cuddle? Who barked? What did the mouse do?\anej{think about if this should be moved forward}

\end{example}

\begin{example}{Long-term dependency in formal language}{long-term-dependency-fl}
    Consider the language $\lang = \{ a b^n a \mid n \in \N \} \cup \{ c b^n c \mid n \in \N \}$.
    Does the string \textexample{$a b^n c$} belong to the language?
    % When reading the last input symbol $a$ of $\strs$, $\rnn$ must recall the initial symbol $a$ of $\strs$.
\end{example}
To be able to answer these questions, a language model must capture \defn{long-term dependencies}\index{long-term dependency}---the relationships between words that are separated by many other words.
How to model such dependencies has long been a key issue for language models.
We have already shown that RNNs have the ability to model inputs of unbounded length.
Yet, this ability should not be taken for granted. It is to be learned from data with considerable effort.

In most cases, we have specifically chosen the dynamics map $\dyMap$ so that the function is \emph{differentiable}.
Because following the gradient of the model's log-likelihood with respect to the parameters is a useful search technique for finding a good model, it is worthwhile to understand how the gradient behaves.
Unfortunately, the gradient of an Elman network is a particularly unstable quantity.
As a function of the length of a training exemplar, in most cases, it tends to either zero or infinity.
This fact, known as the \defn{vanishing and exploding gradient problem}\index{vanishing gradient}\index{exploding gradient}, respectively, is the motivation for many improvements to the Elman network.


In the following discussion, we analyze the gradient behavior of the parameters of an RNN using a generic differentiable $\loss \colon  \paramspace \times \paramspace \rightarrow \Rnonnegative$ as the training objective, denoting $\modelparams$ as some learnable parameters in the RNN.
Vanishing/exploding gradient refers to the cases in which $\frac{\partial \loss}{\partial \modelparams}$ is consistently close to $\zero$ or extremely large in scale, regardless of the input training exemplar.
It is important to keep in mind that vanishing/exploding gradient is different with the extreme gradients on parameters when the model receives clich\'e or unexpected input---the latter one is desirable for training while the former one is not.


Before we start, a few assumptions must be made for our analysis to be meaningful.
\begin{fact}{RNN loss function}{rnn-loss}
    The loss function $\loss$ of an RNN can be written as a function of $\vhzero, \vhone, \cdots, \vhT, \embedMtx$---the sufficient statistics of an input sequence $\str$.
    \begin{align*}
        \loss(\modelparams, \modelparamstrue) \defeq \loss(\vhzero, \vhone, \cdots, \vhT, \embedMtx)
    \end{align*}
    Therefore, its gradient with regard to the parameters $\modelparams$ can be decomposed using the following application of the chain rule:
    \begin{align} \label{eq:rnn-loss-gradient}
        \frac{\partial \loss}{\partial \modelparams} = \sum_{\tstep=0}^{\strlen} \frac{\partial \loss}{\partial \vht} \frac{\partial \vht}{\partial \modelparams} +  \frac{\partial \loss}{\partial \embedMtx}\frac{\partial \embedMtx}{\partial \modelparams}
    \end{align}
\end{fact}
The reasoning behind this fact is that the hidden states $\vhzero, \vhone, \cdots, \vhT, \embedMtx$ are \emph{sufficient} for modeling any desired output given $\str$---they have taken all of the input string and the learned parameters of the model into consideration.
In the context of language modeling, this fact can be rephrased into \emph{``$\vhtminus$ and $\embedMtx$ are the sufficient statistics for $ \pLNSM(\symt \mid \strlt) = \model(\symt \mid \strlt) $---the likelihood of the symbol $\symt$''}(cf. \cref{def:recurrent-neural-language-model}, the $\softmax$ for modeling the distribution of $\symt$ only takes $\vhtminus$ and $\embedMtx$ as input\footnote{This conclusion follows by Neyman-Fisher factorization theorem \citep{neyman-fisher}, since the conditional likelihood can be represented as $\model(\symt \mid \strlt) = \premodel(\vhtminus, \embedMtx)$. }).



In \cref{eq:rnn-loss-gradient}, the term $\frac{\partial \loss}{\partial \vht}$ is a gradient of a one-time application of the loss function, which is stable and easy to evaluate.
Then, we can narrow the scene of vanishing/exploding gradient down to the computation of $\frac{\partial \vht}{\partial \modelparam}$.

% \tianyu{get back to the formal language example. $\symone = a, \cdots \symT = a$, and $\vhone$ is the sufficient statistics for $\symone$}

Without loss of generality, let us look at the case when $\tstep = \strlen$.
$\frac{\partial \vhT}{\partial \modelparam}$ can be further expanded into
\begin{align*}
    \frac{\partial \vhT}{\partial \modelparam}
     & = \frac{\partial \vfunc(\vhTminus, \symT)}{\partial \modelparam}                                                                                                                                                                                                                             \\
     & = \frac{\partial \vhT}{\partial \vhTminus} \frac{\partial \vhTminus}{\partial \modelparam} +  \frac{\partial_{\bar{\vh}} \vhT}{\partial \modelparam}                                                                                                                                         \\
     & = \frac{\partial \vhT}{\partial \vhTminus} \left( \frac{\partial \vhTminus}{\partial \vh_{\strlen-2}} \frac{\partial \vh_{\strlen-2}}{\partial \modelparam} +  \frac{\partial_{\bar{\vh}} \vhTminus}{\partial \modelparam} \right) +  \frac{\partial_{\bar{\vh}} \vhT}{\partial \modelparam} \\
     & = \cdots                                                                                                                                                                                                                                                                                     \\
     & = \sum_{\tstep=0}^{\strlen} \left(\prod_{i=\tstep+1}^{\strlen} \frac{\partial \vhi}{\partial \vhiminus} \right) \frac{\partial_{\bar{\vh}} \vht}{\partial \modelparam}                                                                                                                       \\
     & = \sum_{\tstep=0}^{\strlen}  \frac{\partial \vhT}{\partial \vht} \frac{\partial_{\bar{\vh}} \vht}{\partial \modelparam}
\end{align*}
$\frac{\partial_{\bar{\vh}} \vhT}{\partial \modelparam}$ refers to the partial derivative of $\vhT = \vfunc(\vhTminus, \symT)$ w.r.t. $\modelparam$, while treating $\vhTminus$ as a constant. I.e., the gradient does not backpropagate into $\vhTminus$.
Just like $\frac{\partial \loss}{\partial \vht}$ in \cref{eq:rnn-loss-gradient}, $\frac{\partial_{\bar{\vh}} \vhT}{\partial \modelparam}$ is the derivative of an one-time application of a function, which is easy to evaluate.

%A common and serious problem haunts the training of such neural networks using backpropagation.
\ryan{tie this into the previous notation for loss that Clara wrote.\response{tianyu} Made an assumption on the loss.}
%Conventionally, people take $\vhT$, the hidden state of $\rnn$ after reading the last symbol of the input, as the representation of the whole sequence.
%An objective function $\loss$ then takes $\vhT$ as input.
%Denoting, the $i$-th column vector of $\Jacobianhzero$ as $\vv_i$, the final gradient for $\vhzero$ is $\frac{\partial \loss}{\partial \vhzero} =\left(  \frac{\partial \loss}{\partial \vhT}\right)^{\top} \Jacobianhzero = \left( \inner{\frac{\partial \loss}{\partial \vhT}}{\vv_i} \right)_{i \in \{1,2,\cdots,\hiddDim \}}$.
\ryan{
    Explain two things:
    \begin{itemize}
        \item First, according to the chain rule why $\Jacobianhzero$ pop up and where
        \item Second, the choice of $\vh_0$ is arbitrary. It could have between any two hidden states that are $T$ steps apart.
    \end{itemize}
}

\ryan{Explain what the Jacobian is in more detail. \response{tianyu} refer readers to section:param-estimation}

\tianyu{introducing the idea of `influence function', the influence of $\vhzero$ on $\vhT$. what is vanishing? The influence function! What is exploding? The gradient on the parameters.}

On the contrary, the deeply nested $\frac{\partial \vhT}{\partial \vht}$ can be very unstable.
Mathematically speaking, an RNN is little more than a composition function.
It functions by repeatedly applying the same dynamics map on the hidden state at each time step.

Consider $T$ applications of an RNN's dynamics maps
\begin{equation*}
    \vhT = \dyMap \left( \cdots \dyMap \left(\vhzero, \symone \right) \ \cdots , \symT  \right)
\end{equation*}
Recall \cref{ex:long-term-dependency-fl}, when deciding whether \textexample{$a b^n c$} belongs to $\lang = \{ a b^n a \mid n \in \N \} \cup \{ c b^n c \mid n \in \N \}$ or not, the equation above is instantiated to
\begin{equation*}
    \vhT = \dyMap ( \cdots \underbrace{\dyMap \left(\vhzero, {a} \right)}_{\vhone} \ \cdots , {c} )
\end{equation*}
The decision can only be made after $\rnn$ reads the last symbol $\symT = c$, i.e., when computing $\vhT$.
And most importantly, the computation of $\vhT$ should take the initial symbol $\symone$ into account---$\symone = a$ or $\symone = c$ matter a lot.

We use the sufficient statistics $\vhone$ as the proxy of $\symone$.
And examine how much $\vhT$ is affected when $\vhone$ changes.
The computation of $\vhT$ can be regarded as a vector-valued function, in which $\vhone$ is a variable.
We are interested in the Jacobian $\frac{\partial \vhT}{\partial \vhone}$, which is the best linear approximation of the change in $\vhT$ when giving a small perturbation to $\vhone$. Mathematically speaking, we have
\begin{equation*}
    \Delta \vhT \approx  \frac{\partial \vhT}{\partial \vhone} \Delta \vhone % \lim_{\Delta \vhone \ll 1}
\end{equation*}
With the Jacobian matrix, we can now \emph{quantitatively} analyze long-term dependency.

Again, without loss of generality, we analyze $\frac{\partial \vhT}{\partial \vhzero}$ to get a sense of the gradient effects of long-distance dependencies between hidden states.

Now that we have located the
Vanishing/exploding gradient arises when the $\normlp$-norm $\matNormP{\Jacobianhzero}$ being almost $0$ or extremely large---when it's $0$, long-distance dependencies are not reflected in the gradient updates;
when it's extremely large, long-distance dependencies are overemphasized in at least one dimension.
One term in \cref{eq:rnn-loss-gradient}, the gradient on some parameter $\modelparam$:
\begin{equation*}
    \frac{\partial \loss}{\partial \vhT} \Jacobianhzero \frac{\partial \vhzero}{\partial \modelparam}
\end{equation*}
could be extremely unstable to evaluate. Because an overflow is likely to happen while computing the matrix-vector product.
% {\matNormP{\frac{\partial \vhzero}{\partial \modelparam}}}

% = \max_{i\in\{1,2,\cdots,\hiddDim\}} \matNormOne{\vv_i}
% And the problem worsens when the input length grows. %, as implied by the chain rule decomposition, 
% \begin{align} \label{eq:jacobian-t-to-zero}
%     \Jacobianhzero
%     &= \prod_{\tstep=1}^{\strlen} \Jacobianhtminus 
% \end{align}


We aim to bound the $\normlone$-norm $\matNormOne{\Jacobianhzero}$ from above and below in the following discussions.
The $\normlone$-norm is defined as follows
\begin{definition}[Matrix $\normlone$-norm]
    Suppose $\mA \in \R^{\hiddDim \times \hiddDim}$ with column vectors $\{\vv_i\}_{i = 1,2,\cdots,\hiddDim}$, the $\normlone$-norm of $\mA$ is defined as
    \begin{equation}
        \matNormOne{\mA} = \max_{i \in \{1,2,\cdots,\hiddDim\}} \matNormOne{\vv_i}
    \end{equation}
\end{definition}

In theory, any norm could work for our discussion.
But $\normlone$-norm makes it easier for us to derive the results for the lower bound (\cref{lem:det-normone-inequality}).
For vanishing or exploding gradient, we will respectively give the sufficient condition for the upper bound to \emph{decrease} exponentially or the lower bound to \emph{grow} exponentially.



\begin{theorem}[Vanishing Gradient] \label{thm:vanishing-gradient}
    Suppose the $\normlone$-norm of the Jacobian $\matNormOne{\Jacobianhtminus} \leq C < 1$ is bounded above by a constant, itself less than 1.
    Then $\matNormOne{\Jacobianhzero}$ decreases to $\zero$ exponentially.
\end{theorem}

\begin{proof}
    % \subsubsection{Upper bound on $\matNormOne{\Jacobianhzero}$}
    \cref{thm:vanishing-gradient} is a direct consequence of the matrix norm submultiplicativity:
    \begin{equation} \label{eq:upper-bound-jacobianhzero}
        \normsubone{\Jacobianhzero}
        = \normsubone{\prod_{\tstep=1}^{\strlen} \Jacobianhtminus}
        \le \prod_{\tstep=1}^{\strlen} \normsubone{\Jacobianhtminus}
    \end{equation}

    Suppose $\matNormOne{\Jacobianhtminus} \leq C < 1$, we have
    \begin{equation}
        \normsubone{\Jacobianhzero}
        \le \prod_{\tstep=1}^{\strlen} \normsubone{\Jacobianhtminus} \le C^\strlen
    \end{equation}
    which decreases to $\zero$ exponentially.
\end{proof}


Now, let's turn to another extremity of gradient behaviors.
\begin{theorem}[Exploding Gradient] \label{thm:exploding-gradient}
    Suppose the determinant of the Jacobian $\determinant{\Jacobianhtminus} \geq C > 1$ is bounded below by a constant, itself greater than 1.
    Then $\matNormOne{\Jacobianhzero}$ increases to $\infty$ exponentially.
\end{theorem}

% \subsubsection{Lower bound on $\matNormOne{\Jacobianhzero}$}

The proof of \cref{thm:exploding-gradient} is a bit trickier than the one of \cref{thm:vanishing-gradient}.
To begin with, there is no inequality at hand for us to give a lower bound to the norm of a matrix product.

However, recall the multiplicativity of determinant: $\determinant{\mA\mB} = \determinant{\mA}\determinant{\mB}$ for square matrices $\mA, \mB$.
It hints that the determinant can be used as a bridge in lower bounding the product of $\Jacobianhtminus$.
Meanwhile, the determinant itself can serve as a lower bound for the $\normlone$-norm by the following inequality:
\begin{fact}{Hadamard's Inequality}{hadamard-inequality}
    The following inequality holds for $\mA \in \R^{\hiddDim \times \hiddDim}$ with column vectors $\{\vv_i\}_{i = 1,2,\cdots,\hiddDim}$
    \begin{align}
        \determinant{\mA} \le \prod_{i=1}^{\hiddDim} \normsubtwo{\vv_i}
    \end{align}
    The equality is achieved if and only if  $\vv_i$ are orthogonal. For detailed proof, we refer the readers to \citet[Corollary 7.8.3]{horn2013}.
\end{fact}

By \cref{fact:hadamard-inequality}, we can bound the $\normlone$-norm of a matrix $\mA$ from below using its determinant $\determinant{\mA}$.
\begin{lemma}{Determinantal lower bound on matrix $\normlone$ norm}{det-normone-inequality}
    Let $\mA \in \R^{\hiddDim\times\hiddDim}$, we have
    \begin{align*}
        \determinant{\mA} \le \normsubone{\mA}^{\hiddDim}
    \end{align*}
\end{lemma}

\begin{proof}
    Let $\mA \in \R^{\hiddDim\times\hiddDim}$, we have
    \begin{align}
        \determinant{\mA}
         & \le \prod_{i=1}^{\hiddDim} \normsubtwo{\vv_i}  \tag{\text{Hadamard's inequality}}    \\
         & \le \prod_{i=1}^{\hiddDim} \normsubone{\vv_i} \tag{\text{Cauchy-Schwarz inequality}} \\
         & \le \normsubone{\mA}^{\hiddDim} \tag{\text{Property of $\normlone$ norm}}
    \end{align}
    The first equality is achieved if and only if $\vv_i$ are orthogonal.
    The second equality is achieved if and only if $\vv_i$ are $\zero$ or parallel with standard basis vectors.
    The third equality is achieved if and only if all $\matNormOne{\vv_i}$ are the same.
\end{proof}

Note that when $\determinant{ \mA } \le 0$, \cref{lem:det-normone-inequality} becomes a trivial inequality $\normsubone{\mA} \ge 0$.


With \cref{lem:det-normone-inequality}, we can now present the proof for \cref{thm:exploding-gradient}:

\begin{proof}[Proof of \cref{thm:exploding-gradient}]
    By \cref{lem:det-normone-inequality}, we give a lower bound on $\matNormOne{\Jacobianhzero}$:
    \begin{align} \label{eq:lower-bound-jacobianhzero}
        \normsubone{\Jacobianhzero}
         & \ge \left( \determinant{\Jacobianhzero} \right)^{\frac{1}{\hiddDim}} \nonumber                            \\
         & = \left( \determinant{\prod_{\tstep=1}^{\strlen} \Jacobianhtminus} \right)^{\frac{1}{\hiddDim}} \nonumber \\
         & =  \prod_{\tstep=1}^{\strlen} \left( \determinant{ \Jacobianhtminus } \right)^{\frac{1}{\hiddDim}}
    \end{align}

    Suppose $\determinant{\Jacobianhtminus} \geq C > 1$, we have
    \begin{equation*}
        \normsubone{\Jacobianhzero} \ge C^{\frac{\strlen}{\hiddDim}}
    \end{equation*}
    which increases to $\infty$ exponentially as $\strlen \to \infty$ .
\end{proof}

Combining the upper bound (\cref{eq:upper-bound-jacobianhzero}) and the lower bound (\cref{eq:lower-bound-jacobianhzero}), we have:
\begin{corollary}{}{bounded-jacobianhzero}
    $ \normsubone{\Jacobianhzero} $ satisfies the following inequalities:
    \begin{equation}
        \prod_{\tstep=1}^{\strlen} \left( \determinant{ \Jacobianhtminus } \right)^{\frac{1}{\hiddDim}} \le \normsubone{\Jacobianhzero} \le \prod_{\tstep=1}^{\strlen} \normsubone{\Jacobianhtminus}
    \end{equation}
\end{corollary}

Up to this point, we have concluded our analysis of the gradient of RNNs.
A hot takeaway is that gradient-based optimization can be extremely unstable for long-term dependencies.
We must carefully choose the dynamics map $\dyMap$ so as to avoid the vanishing/exploding gradient conditions.

To understand how \cref{thm:vanishing-gradient,thm:exploding-gradient} matter in practice, let us take the Elman sequence model as an example to instantiate the above bounds. Recall its dynamics map $\dyMap$:
\begin{align}
    \hiddStateZero & = \zero                                                                                                             & \nonumber    \\
    \vht           & = \dyMap(\vhtminus, \symtminus) = \sigmoid\!\left( \recMtx \vhtminus + \inMtx \inEmbedSymtminus + \biasVech \right) & \tstep \ge 1
\end{align}
where $\sigmoid$ is a non-linearity applied to the input element-wise. The step-wise gradient for one step of hidden state update is:
\begin{align}
    \Jacobianhtminus
     & = \frac{\partial \dyMap(\vhtminus, \symtminus)}{\partial \vhtminus} \nonumber                                          \\
     & = \diag{\sigmoidVecPrime{}\!\left( \recMtx \vhtminus + \inMtx \inEmbedSymtminus + \biasVech \right)} \recMtx \nonumber \\
     & \defeq \diag{\sigmoidVecPrime{\tstep}} \recMtx
\end{align}

\begin{fact}{A fact about the Jacobian matrix}{elman-bounded-jacobianhzero}
    For Elman networks, $ \normsubone{\Jacobianhzero} $ satisfies the following inequalities
    \begin{equation}
        \prod_{\tstep=1}^{\strlen} \left( \determinant{ \diag{\sigmoidVecPrime{\tstep}} \recMtx} \right)^{\frac{1}{\hiddDim}} \le \normsubone{\Jacobianhzero} \le \prod_{\tstep=1}^{\strlen} \normsubone{\diag{\sigmoidVecPrime{\tstep}} \recMtx}
    \end{equation}
\end{fact}
\subsubsection{Vanishing Gradient}
To find out when vanishing gradient could happen, we aim to find the $\diag{\sigmoidVecPrime{\tstep}} \recMtx$ that makes the upper bound decrease exponentially with the length of the input.


The derivative of activation function $\sigmoidVecPrime{}$ is bounded in many cases (e.g., $\ReLU$, $\text{sigmoid}$).
Denoting $\constbound$ as the upper bound such that $ \forall \evx \in \R, |\sigmoidVecPrime{}(\evx) | \le  \constbound$, we have
\begin{align}
    \normsubone{\frac{\partial \vhT}{\partial \vhzero}}
     & \le \left( \constbound \normsubone{\recMtx} \right)^\strlen
\end{align}

% This inequality shows that $\constbound \normsubone{\recMtx} < 1$ is the \emph{sufficient} condition for vanishing gradient.
The term $ \left(\constbound \normsubone{\recMtx}\right) ^\strlen$ exponentially shrinks to $0$ when $\constbound \normsubone{\recMtx} < 1$.
The hidden states corresponding to the earlier part of the input sequence will receive very limited gradient updates.


\subsubsection{Exploding Gradient}

A weaker result can immediately be derived by inverting the proof for the upper bound:
$\constbound \normsubone{\recMtx} \geq 1$ is the \emph{necessary} condition for exploding gradient.
Since otherwise, the gradient would vanish.

However, we are not satisfied with this conclusion.
By \cref{fact:elman-bounded-jacobianhzero}, we present a sufficient condition that leads to exploding gradient\footnote{Our analysis does not make assumptions on the choice of non-linearity, which makes itself more general than the analysis of \citet{pascanu-rnn} that assumes identity activation.}.

\begin{align}\label{eq:lower-bound-exploding-gradient}
    \normsubone{\Jacobianhzero}
     & \ge \left( \prod_{\tstep=1}^{\strlen} \determinant{\diag{\activprimet}} \determinant{\recMtx} \right)^{\frac{1}{\hiddDim}}
    % &=  \left( \determinant{\recMtx} \right)^{\frac{\strlen}{\hiddDim}}  \prod_{\tstep=1}^{\strlen}  \determinant{\diag{\activprimet}}^{\frac{1}{\hiddDim}} \nonumber 
\end{align}

When $\frac{\strlen}{\hiddDim}$ is sufficiently large, and $\determinant{\recMtx} \determinant{\diag{\activprimet}} > 1$, an exploding gradient will appear.

For instance, let the activation function $\sigmoid = \ReLU$, $\recMtx \vht + \inMtx \inEmbedSymt + \biasVech > 0 \ \text{for all } \tstep\ge1$, and $\determinant{\recMtx} = \constbound > 1$.
Then, $\determinant{\diag{\activprimet}} = 1$, for all $\tstep \in \{1, 2, \cdots, \strlen \}$.
We have
\begin{align}\label{eq:upper-bound-exploding-gradient}
    \normsubone{\Jacobianhzero}
     & \ge \constbound^{\frac{\strlen}{\hiddDim}}
    % &=  \left( \determinant{\recMtx} \right)^{\frac{\strlen}{\hiddDim}}  \prod_{\tstep=1}^{\strlen}  \determinant{\diag{\activprimet}}^{\frac{1}{\hiddDim}} \nonumber 
\end{align}
which exponentially increases to $\infty$ as $\strlen \to \infty$.


\subsubsection{Why is vanishing/exploding gradient a problem?}
The computing frameworks we employ to implement a language model often have finite precision.
The parameters and intermediate variables during computing are represented by floating-point numbers, among which \fpfull{} is most commonly used.

The minimal value above zero that a \fpfull{} number can represent is \num{1.2e-38}, while the maximal is \num{3.4e+38}.
All values outside this range will be truncated to one of the three values: $0$, $\textnormal{NaN}$, or $\textnormal{inf}$.



When vanishing gradient appears, gradient signals from long-term dependencies are extremely small in scale.
% since they are far smaller in scale than those for nearby inputs. 
Gradient signals could also be rounded off to zero due to the finite float precision.
When making decisions, the trained model tends to lose track of long-distance dependencies and only relies on the nearest neighbors of the hidden states $\vht$ it chooses to use.
On the other hand, a gradient that is too large in scale could lead to $\textnormal{NaN}$ updates during training, interrupting the training process.
% Even if such an error does not happen, the former part of the input sequences will receive more updates than the latter.
% When making decisions, the trained model tends to rely on the input's \emph{former} part. 

In \cref{sec:var-rnn}, we will discuss some techniques for countering vanishing/exploding gradient.



==> chapters/neural-lms/variations_transformer.tex <==
A significant disadvantage of the transformer architecture is the quadratic time and space complexity of its attention mechanism with respect to the length of the input sequence. The quadratic complexity of the attention layer arises from the matrix multiplication between $\mQ$ and $\mK$ in~\cref{eq:attention_block}. This operation runs in $\mathcal{O}(\tfslen^2 \hiddDim)$. The quadratic complexity of attention makes transformers less scalable, and prevents their use in tasks that require, or would benefit from, supporting long input sequences. To overcome this limitation, many modifications to the original architecture were proposed after the publication of the original transformer. These efficient variants of transformers are generally called \defn{efficient transformers} and improve on the architectural limitations of transformers using a wide variety of different methods. Here we present a brief overview before explaining two efficient transformer models in more detail.

The earliest and simplest modifications of self-attention sparsify the attention matrix by limiting the tokens to attend to limited, \textbf{fixed patterns}. Multiple pattern types are possible: blockwise patterns chunk the input sequence into fixed blocks, and compute attention only within each block. Strided patterns only attend to tokens positioned at fixed distance intervals. Alternatively, compressed patterns are obtained by applying a pooling operator, such as a convolution, to downsample $\mQ$ or $\mK$ and obtaining a smaller matrix. Multiple fixed patterns can be combined into a single attention variant in an effort to improve the its overall coverage. For instance, Big Bird~\citep{Zaheer2020BigBird}, whose attention matrix is shown in~\cref{fig:bigbird_attention} combines a strided pattern with random attention, limiting the computation of full attention only to a limited amount of symbols. These patterns don't necessarily need to be fixed, but can also be learned jointly with the rest of the model parameters. In practice, \textbf{Learnable patterns} aim to cluster input tokens based on their relevance for one another. Clustering can be achieved through the use of a similarity function that is trained jointly with the rest of the network in a data-driven manner. Other methods that don't rely on patterns to make the attention matrix more sparse are also adopted: \textbf{Low-Rank Methods} apply low-rank approximations to reduce the size of $\mQ$ or $\mK$ assuming that the attention matrix $\mA$ has low rank. Alternatively, \textbf{kernels} can be used to encode the $\softmax$ function and sidestep matrix multiplication between queries and keys. 

In the rest of the section, we will analyze two efficient transformer architectures that improve the complexity of the attention mechanism with different approaches.


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/bigbird_attention.png}
    \caption{BigBird combines random attention (a), strided attention (b), and global attention (c) to obtain a sparse attention matrix (d). Image source: ~\cite{Zaheer2020BigBird}.}
    \label{fig:bigbird_attention}
\end{figure}

\subsubsection{Sparse Transformer}
The Sparse Transformer~\citep{child2019sparsetransformer} is an efficient transformer architecture that relies on fixed patterns to sparsify the attention matrix. The time complexity of the Sparse Transformer is $\mathcal{O}(\tfslen\sqrt{\tfslen})$. 
\clara{would be nice if this were presented the same way as how attention is first introduced}
We start by rewriting~\cref{eq:single_query_attn_score} as:
\begin{equation}\label{eq:reformer_single_query_attn}
    s_i = \sum_{j \in \mathcal{P}_i}{\exp{(\vq_i \cdot \vk_j} - \rz(i, \mathcal{P}_i)})\vv_j \qquad \text{where } \mathcal{P}_i = \{j: j \leq i\}
\end{equation}
where we denote with $\rz(i, \mathcal{P}_i)$ the normalization term of the $\softmax$. The set $\mathcal{P}_i$ prevents the token at input $i$ to attent to future tokens. Our goal is to find \defn{attention subsets} $\mathcal{A}^{(h)}_i \subset \mathcal{P}_i$ so that $|\mathcal{A}_i^{(h)}| \propto \sqrt{\tfslen}$. We can restrict the search for $\mathcal{A}_i^{(h)}$ to consider only fully-connected choices.
Fully-connected attention subsets are capable of propagating signals from arbitrary positions to arbitrary positions in $N$ attention blocks. 
\begin{definition}[Fully-connected attention subsets]
    $N$ attention subsets are said to be \defn{fully-connected} if $\ \forall i, j: 0\leq j \leq i < \tfslen$ there exists a sequence of indices $(j, n_1, n_2, \dots, n_N, i)$ for which the following holds.
    \begin{equation}
        j \in \mathcal{A}_{n_1}^{(1)}, n_1 \in \mathcal{A}_{n_2}^{(2)}, \dots, n_N \in \mathcal{A}_{i}^{(N)}
    \end{equation}
\end{definition}
Each attention subset can either be assigned to a different head in the same attention block, or be computed separately in two sequential attention blocks. We introduce two alternative definitions of fully-connected subsets for $N=2$.
The first method is called \defn{strided attention} and is obtained by using attention subsets defined as follows.
\begin{align}
    &\mathcal{A}_i^{(1)} = \{k, k+1, \dots, i\} \text{ for } k = \max(0, i-\tfslen) \text{ and } 0\leq i < \tfslen\\
    &\mathcal{A}_i^{(2)} = \{j: (i-j)\mod{\tfslen} = 0\}
\end{align}
Strided attention is particularly useful if the data under consideration has a periodic structure. 
Alternatively, we can define \defn{fixed attention} by using the following attention subsets.
\begin{align}
    &\mathcal{A}_i^{(1)} = \{j, (\lfloor j/\tfslen\rfloor =\lfloor i/\tfslen\rfloor )\} \\
    &\mathcal{A}_i^{(2)} = \{j:j\mod{\tfslen} \in \{\tfslen-c, \tfslen-c+1, \tfslen-c+2, \dots, \tfslen\}\}
\end{align}
The two patterns are visualized in~\cref{fig:sparse_transformer}. 

\begin{figure}[h]
\centering
    \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/strided-attn.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/fixed-attn.png}
    \end{subfigure}
    \caption{Visualizations of the attention matrix using the patterns encoded by strided attention (left) and fixed attention (right). Blue and light blue squares indicate the positions covered by the two attention subsets. Grey squares are ignored, sparsifying the matrix. Image source:~\cite{child2019sparsetransformer}}
    \label{fig:sparse_transformer}
\end{figure}


\subsubsection{Reformer}
The Reformer~\citep{Kitaev2020Reformer} is an efficient transformer architecture that improves the time and memory complexities of attention using learnable patterns. Specifically, the Reformer replaces dot-product attention with Locality Sensitive Hashing (LSH) attention, obtaining a complexity of $\mathcal{O}(\tfslen \log \tfslen)$. 

We start by rewriting~\cref{eq:single_query_attn_score} as:
\begin{equation}\label{eq:reformer_single_query_attn}
    s_i = \sum_{j \in \mathcal{P}_i}{\exp{(\vq_i \cdot \vk_j} - \rz(i, \mathcal{P}_i)})\vv_j \qquad \text{where } \mathcal{P}_i = \{j: j \leq i\}
\end{equation}
where we denote with $\rz(i, \mathcal{P}_i)$ the normalization term of the $\softmax$. 

We can reformulate~\cref{eq:reformer_single_query_attn} by using a larger set $\tilde{\mathcal{P}}_i := \{0, 1, \dots, \tfslen\}$ to draw keys and values from, and make the masking explicit by zeroing out unnecessary elements that are not contained in $\mathcal{P}_i$ as follows:

\begin{align}\label{eq:reformer_masked_attention}
    &s_i = \sum_{j \in \tilde{\mathcal{P}}_i}{\exp{(\vq_i \cdot \vk_j} - m(j, \mathcal{P}_i) - \rz(i, \mathcal{P}_i)})\vv_j \\
    &\text{where } m(j, \mathcal{P}_i) = \begin{cases} \infty \quad \text{if } j \notin \mathcal{P}_i \\ 0 \quad \text{otherwise} \end{cases}\nonumber
\end{align}

In LSH attention, we define $\mathcal{P}_i$ as follows:
\begin{equation}\label{eq:reformer_bucket_equality}
    \mathcal{P}_i = \{j: h(q_i) = h(k_j) \} 
\end{equation}
where $h(\cdot)$ is a hashing function. Therefore, the attention between a query and a key is not masked out only if the query and the key have the same hash. We aim to approximate the output of the $\softmax$ function over the attention matrix by considering, for each query $\vq_i$, only the subset of keys that are closer to it, i.e. the keys that yield the higher scores $s_{ij} = \vq_i^{\top}\vk_j$. We rely on Locality-Sensitive Hashing to find this subset of keys. LSH is a hashing scheme that assigns the same hash to vectors that are closer together with high probability. Here, we define the LSH hash function $h(\cdot)$ as follows:
\begin{equation}\label{eq:reformer_lsh_hashing}
    h(\vx) = \operatorname{argmax}([\vx\mR ; -\vx\mR])
\end{equation}
where $\mR \in \R^{\ell \times b/2}$, $b$ is the number of buckets that the input vector can be assigned to, and $[\vu; \vv]$ denotes vector concatenation. 

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/reformer_LSH_chunks.png}
    \caption{Depiction of LSH attention from~\cite{Kitaev2020Reformer}.}
    \label{fig:reformer_lsh}
\end{figure}

Using LSH in this form on both queries and keys can have two adverse effects: the number of keys or queries per hash bucket has high variance, and the number or queries in a hash bucket can differ from the number of keys in the same bucket. Both these issues can make computing LSH attention more complicated. To avoid these issues, each key is set to be equal to its corresponding normalized query $\vk_j = \frac{\vq_j}{||\vq_j||}$. In practice, this is achieved by setting the key projection matrix $\mW_k$ to be equal to the query projection matrix $\mW_q$ and normalizing its rows. A transformer model having keys equal to its queries is called \defn{shared-QK transformer}. While this setting reduces the number of parameters of the transformer and could therefore worsen its performance, it is verified in practice that the difference in performance between a shared-QK transformer and the full architecture is negligible. 

After hashing, queries are sorted by bucket number and, within each bucket, by position in the input sequence. The sorting procedure defines a permutation $i \mapsto s_i$ where $i$ is the position of $\vq_i$ before sorting, and $s_i$ after sorting. The sorted queries are split into chunks of $m$ consecutive elements where $m$, the chunk size, is fixed as $m = \frac{2\tfslen}{b}$. Each query is then allowed, only within the bucket to which it belongs, to attend to keys in the same or in the previous chunk. This corresponds to defining $\tilde{\mathcal{P}}_i$ as follows.

\begin{equation}\label{eq:reformer_chunking}
    \tilde{\mathcal{P}}_i = \left\{ j: \left\lfloor \frac{s_i}{m} \right\rfloor - 1 \leq  \frac{s_j}{m} \leq \left\lfloor \frac{s_i}{m} \right\rfloor \right\}
\end{equation}

The LSH attention method is shown graphically in~\cref{fig:reformer_lsh}.~\Cref{eq:reformer_chunking} restricts the allowed keys to come from either the same or the previous chunk as the one that contains the current query, while ~\cref{eq:reformer_bucket_equality} performs the bucket masking, filtering out all keys that don't belong to the same bucket as the current query. Since the masking in~\cref{eq:reformer_masked_attention} now operates over the hash buckets, we need to implement the autoregressive property and prevent tokens from peeking into the future using another method. This is achieved by associating every query with a position index and reordering the position indices with the same permutation. An additional mask is then used to only allow valid positions. Contrary to ordinary masked attention, LSH attention additionally prevents each query to attend to itself, since, due to QK-sharing, the dot product of a query vector with itself will always be higher than the dot product with any other token. This restriction is only lifted where the query tokens has no other tokens to attend to except for itself, for example, at the beginning of the string.
% While the hash function guarantees by definition to associate nearby tokens with high probability, we can reduce the probability that different tokens fall in the same hash bucket by doing multiple hashing rounds, i.e. performing hashing multiple times, obtaining:

% \begin{align}
%     &\mathcal{P}_i = \bigcup_{r=1}^{n_{rounds}}{\mathcal{P}^{(r)}} \\
%     &\text{where } \mathcal{P}^{(r)} = \{ j: h^{(r)}(\vq_i) = h^{(r)}(\vq_j) \}\nonumber
% \end{align}

% source: https://openreview.net/forum?id=rkgNKkHtvB&noteId=Byx13YvZOB
We now analyze the time complexity of LSH attention. The complexity can be split into two parts: the complexity of computing attention between chunks, and the complexity of performing the hashing. The attention complexity can be computed as follows: each sequence of length $\tfslen$ is split into chunks of length $m = \frac{\tfslen}{b}$, where $m$ is set to a constant value. Each of the $\frac{\tfslen}{m}$ chunks performs attention of size $m \times 2m$, where the 2 comes from the fact that each token can attend to both its own chunk and the previous one. Therefore, we have:

\begin{align}
    &\mathcal{O}\left(\frac{\tfslen}{m}(2m^2)\right) = \mathcal{O}\left(\frac{2\tfslen}{m}\left(\frac{4\tfslen^2}{b^2}\right)\right) = \mathcal{O}\left(b\left(\frac{2\tfslen}{b}\right)^2\right) = \nonumber \\
    &=\mathcal{O}\left(\frac{4\tfslen^2}{b}\right) = \mathcal{O}\left(2\tfslen m\right) = \mathcal{O}\left(\tfslen\right)
\end{align}

where the last equality is valid since $m$ is considered a constant. The complexity of performing the hashing of queries and keys is derived from the hashing function in ~\cref{eq:reformer_lsh_hashing}. This hashing function consist of performing two matrix multiplications which take $\mathcal{O}\left(\tfslen\hiddDim\frac{b}{2} \right)$ time each. If we choose $b = \log{(\tfslen)}$ as the number of hash buckets, we obtain $\mathcal{O}(\tfslen\log{\tfslen})$ as the LSH complexity, where $\hiddDim$ is treated as a constant and the $2$ disappears after concatenation. The full complexity of LSH attention is then:

\begin{equation}
    \mathcal{O}(\tfslen\log{(\tfslen)} + \tfslen) = \mathcal{O}(\tfslen\log{(\tfslen}))
\end{equation}

It's worth noting that, while this complexity can seem like a net improvement over the quadratic complexity of standard attention, it does not take into account the large constants hidden by the Big-O notation. In practical use, these constants can limit the actual speed-ups of this architecture over standard full attention. In practice, this makes the Reformer more efficient than the original transformer only when used for extremely long sequences.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LINFORMER  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Linformer}
% The Linformer~\citep{wang2020linformer} is an efficient transformer model that obtains a linear self-attention runtime of $\mathcal{O}(\tfslen)$ by leveraging the fact that the self-attention matrix $\mM \in \R^{\tfslen \times \tfslen}$ is low rank. The low-rank property of the attention matrix is useful because it allows us to approximate it with a truncated matrix $\mA_k$ having $\operatorname{rank(\mA_k)}=k$ using the following theorem.

% \begin{theorem}[Eckart–Young–Mirsky]
%     A matrix $\mA \in \R^{\tfslen \times \tfslen}$ whose Singular Value Decomposition\footnote{https://en.wikipedia.org/wiki/Singular\_value\_decomposition} is $\mA = \mU\mD\mV^{\top}$ can be approximated with matrix $\mA_k = \mU \operatorname{diag}([\sigma_1, \dots, \sigma_k]) \mV^{\top}$ with the following approximation error:
%     \begin{equation*}
%         \|\mA - \mA_k \|_2 = \sigma_{k+1}
%     \end{equation*} 
%     Where $\| \cdot \|_2$ is the spectral norm and $\sigma_k$ is the $k-th$ biggest eigenvalue of $\mA$.
% \end{theorem}

% Therefore, if the $k+1$-th eigenvalue of $\mA$ is small, the approximation error obtained when using $\mA_k$ instead of $\mA$ will be negligible.


% We start by recalling the formulation of (scaled dot-product unmasked) self-attention from~\cref{alg:transformer_attention}:
% \begin{align}\label{eq:linformer_attention}
%     \texttt{Attention}(\mX) &= \softmax \left(\frac{\mX\mW_q^{\top}((\mX\mW_k^{\top})^{\top})}{\sqrt{d_{attn}}}\right) \mX\mW_v^{\top} = \nonumber \\
%     &= \softmax(\mS) \mX\mW_v^{\top} = \mA\mX\mW_v^{\top}
% \end{align}
% where we highlight the score matrix $\mS$ and the attention matrix $\mA$ in the last two steps, respectively.

% We are interested in proving that the the attention matrix $\mA$ is low rank, so that we can approximate it using a low-rank matrix approximation method and reduce the complexity of self-attention. We prove the low-rank property of $\mA$ by making use of the following lemma:

% \begin{lemma}[Johnson-Lindenstrauss~\citep{Johnson1984ExtensionsOL}]\label{lem:johnson-lindenstrauss}
%     Let $\mR \in \R^{k \times n}, 1 \leq k \leq n$ be a matrix with i.i.d. entries sampled from a normal distribution $\mathcal{N}(0, 1/k)$. For any $\vx$, $\vy \in \R^{n}$, we have:
%     \begin{align}
%         & \probfunction\left(||\mR\vx^{\top}|| \leq (1+\epsilon)||\vx||\right) > 1-\exp{\frac{-(\epsilon^2-\epsilon^3)k}{4}} \\
%         & \probfunction\left(||\vx\mR^{\top}\mR\vy^{\top} - \vx\vy^{\top}|| \leq \epsilon||\vx\vy^{\top}\right) > 1-2\exp{\frac{-(\epsilon^2-\epsilon^3)k}{4}}
%     \end{align}
% \end{lemma}

% Using the Johnson-Lindenstrauss lemma, we can prove the following:
% \begin{theorem}[$\mA$ is low rank]
% For any $\mX \in \R^{\tfslen \times d_{in}}$, $\mW_q$, $\mW_k \in \R^{d_{attn} \times d_{in}}$, $\mW_v \in \R^{d_{o}\times d_{in}}$, and any column vector $\bomega \in \R^{\tfslen}$, there exists a low-rank matrix $\tilde{\mP} \in \R^{\tfslen \times \tfslen}$ such that:
% \begin{align*}
%     &\probfunction \left(||\tilde{\mP}\bomega^{\top} - \mP\bomega^{\top}|| < \epsilon ||\mP\bomega^{\top}|| \right) > 1 - o(1) \\
%     &\text{and } \operatorname{rank}(\tilde{\mP}) = \Theta(\log{(\tfslen)})
% \end{align*}
% where $\epsilon > 0$ is the approximation error.
% \begin{proof}
%     We redefine the attention matrix $\mA$ as:
%     \begin{equation}
%         \mA = \exp{(\mS)\mD_A^{-1}}
%     \end{equation}
%     where $\mD_A$ is a diagonal matrix with the following elements:
%     \begin{equation}
%         \mD_A[i, i] = \sum_{j=1}^{\tfslen}{\exp{(S[j, i])}}
%     \end{equation}
%     We define the following matrix:
%     \begin{equation}\label{eq:linformer_approx_a}
%         \tilde{\mA} = \exp{(\mS)} \mD_A^{-1} \mR^{\top}\mR
%     \end{equation}
%     where $\mR \in \R^{k \times \tfslen}$ has the same form as in~\cref{lem:johnson-lindenstrauss}.
%     Due to the multiplication with $\mR$, we have the following regarding the rank of $\tilde{\mP}$:
%     \begin{equation}
%         \operatorname{rank}(\tilde{\mA}) \leq \operatorname{rank}(\mR) = k
%     \end{equation}
%     We now apply~\cref{lem:johnson-lindenstrauss} obtaining, for any row vector $\vu \in \R^{\tfslen}$ of $\mP$, and column vector $\vw \in \R^{\tfslen}$ of $\mX\mW_v^{\top}$:
%     \begin{align*}
%         & \probfunction\left(||\tilde{\mA}\bomega^{\top} - \mA\bomega^{\top}|| < \epsilon ||\mA\bomega^{\top}|| \right) = \\
%         &= \probfunction\left(|| \mA\mR^{\top}\mR\vw^{\top} - \mA\vw^{\top} || \leq \epsilon||\mA\vw^{\top}|| \right) \geq \\
%         &\geq 1 - \sum_{\vx \in \mA}{\probfunction\left(||\vx\mR^{\top}\mR\vx - \vx\vw^{\top}|| - \epsilon ||\vx\vw^{\top} \right)} > \\
%         &> 1 - 2\tfslen\exp{\left(-\frac{-(\epsilon^2 - \epsilon^3)k}{4}\right)} \\
%         &> 1 - o(1)
%     \end{align*}
%     The second linefollows from~\cref{eq:linformer_approx_a}, the third through Boole's inequality\footnote{
%         $p\left(\bigcup_{i=1}^{\infty}{\sE_i}\right) \leq \sum_{i=1}^{\infty}p\left(\sE_i\right)$ for a countable set of events $\sE_1, \sE_2, \dots \in \eventspace$.
%     }, and the fourth using ~\cref{lem:johnson-lindenstrauss}. Finally, we obtain the desired expression in the last line by setting $k = 5\log{(\tfslen)}/(\epsilon^2-\epsilon^3)$
% \end{proof}
% \end{theorem}

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{figures/linformer_spectrum.png}
%     \caption{From~\cite{wang2020linformer}: The largest 128 eigenvalues out of $512 = d_{attn}$ contain more than $90\%$ of the total eigenvalue mass.}
%     \label{fig:linformer_spectrum}
% \end{figure}

% The low-rank property of $\mA$ is also proven empirically by training two encoder-only transformer models on two different classification tasks and performing Singular Value Decomposition (SVD) on all attention matrices.~\cref{fig:linformer_spectrum} shows that for both model sizes, for both tasks, most of the information contained in $\mA$ can be recovered from the largest singular values.

% Knowing that $\mA$ is low rank, we could apply SVD to approximate it, but this approach would require performing SVD separately for each head and each self-attention layer, which would be computational expensive. Therefore, the Linformer adopts a different approach based on adding two additional linear projections $\mE, \mF \in \R^{\tfslen \times k}$ in the computation of keys and values, respectively.~\cref{eq:linformer_attention} is then modified as follows:

% \begin{align}
%     \texttt{Attention}(\mX) &= \softmax \left(\frac{\mX\mW_q^{\top}((\mE\mX\mW_k^{\top})^{\top})}{\sqrt{d_{attn}}}\right) \mF\mX\mW_v^{\top} \nonumber \\
%     &= \bar{\mA}(\mF\mX\mW_v^{\top} )
% \end{align}

% where the first factor in the last line has size $\tfslen \times k$ and the second $\tfslen \times d_{o}$. This formulation of attention has $\mathcal{O}(\tfslenk)$ complexity instead of $\mathcal{O}(\tfslen^2)$, therefore, by leveraging the low-rank property of $\mA$ and using a small $k$, we can approximate $\mA$ with $\bar{\mA}$ we can compute self-attention in linear time. The following theorem guarantees that we can limit the approximation error to $\epsilon$ by choosing $k=\mathcal{O}(d_{o}/epsilon^2)$.

% \begin{theorem}
% For any $\mX \in \R^{\tfslen \times d_{in}}$, $\mW_q$, $\mW_k \in \R^{d_{attn} \times d_{in}}$, $\mW_v \in \R^{d_{o}\times d_{in}}$, if $k=\min\{\Theta(9d_{o} \log(d_{o})/\epsilon^2), 5\Theta(\log(\tfslen)/\epsilon^2)\}$, then there exists matrices $\mE$, $\mF \in \R^{\tfslen \times k}$ such that, for any row vector $\vw$ of \newline $\left(\mX\mW_q^{\top}((\mE\mX\mW_k^{\top})^{\top}/\sqrt{d_{attn}}\right)$ we have:

% \begin{align}
% \probfunction(||\softmax(\vw\mE^{\top})&\mF\mX\mW_v^{\top} - \softmax(\vw)\mX\mW_v^{\top}||  \nonumber\\
% &\leq ||\softmax(\vw)||||\mX\mW_v^{\top}|| ) > 1 - o(1)
% \end{align}
% \end{theorem}

% \begin{proof}
% For ease of notation, we first define matrices $\mQ'=\mQ\mW_q^{\top}$, $\mK'=\mK\mW_k^{\top}$, and $\mV'=\mV\mW_v^{\top}$ and assume that $d_{attn} = d_{o} = d$ so that $\mQ', \mK', \mV' \in \R^{\tfslen \times d}$.

% We define matrix $\mR \in \R^{\tfslen \times k}$ with i.i.d. entries sampled from $\mathcal{N}(0, \frac{1}{k})$, and two matrices derived from $\mR$: $\mE$, $\mF \in \R^{\tfslen \times k}$.

% We start by proving that for any row vector $\vx \in \R^{\tfslen}$ of matrix $\mQ'\mK'^{\top}$ and any column vector $\vy \in \R^{\tfslen}$ of matrix $\mV'$:

% \begin{equation}
% \probfunction\left(\left\|\exp\left(\vx\mE^{\top}\right)\mF\vy^{\top}-\exp(\vx) \vy^{\top}\right\| \leq \epsilon\left\|\exp(\vx) \vy^{\top}\right\|\right)>1-2 e^{-\left(\epsilon^2-\epsilon^3\right)k / 4}

% \end{equation}

% \end{proof}

% The $\mE$, $\mF$ matrices can be then shared across different heads, different layers, or both. It's also possible to use the same projection matrix for both keys and values by setting $\mE = \mF$. Empirical results show that the performance of Linformer does not significantly decrease even when sharing the same projection matrix across the whole architecture.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LONGFORMER %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsubsection{Longformer}
% As the first example of an efficient transformer model, we look at the Longformer~\citep{beltagy2020longformer}, a transformer variant that linearizes the computation of attention by sparsifying the attention matrix using a combination of fixed patterns. In particular, the Longformer computes attention by combining dilated slided window attention and global attention. Assuming that tokens immediately surrounding a token are more important than token far away, sliding window attention only performs attention for tokens at or below a fixed size distance from each token, i.e. given a window size $w$, each token attends to tokens at a maximum distance of $\frac{1}{2}w$ on each side, in a way that is similar to performing a 1D-convolution with kernel size $w$ over the input sequence. This makes the whole computational complexity of computing sliding window attention come to $\mathcal{O}(\tfslen w)$, linear in the input length when choosing small values of $w$. By stacking multiple self-attention layers, the receptive field of each token increases, with the deepest layers being able to reach all tokens in the input sequence for sufficiently high values of $w$. Sliding window attention can then be extended to a dilated version that computes attention as follows.

% \begin{equation}
%     \hat{\mS}_{ij} = \begin{cases}
%         \mQ_i\mK_j^{\top} \quad \text{if } (i-j)\mod d = 0 \\
%         0 \quad \text{otherwise}
%     \end{cases}
% \end{equation}

% In this case, the receptive field of a token is $\tfslen \times w \times d$, where $d$ the parameter controlling the dilation. Different values of $w$, and $d$ can be set for different attention layers: in the Longformer, the window sizes are set to small values for the first layers, and increased in the deeper layers. This allows the first layers to focus on learning the local context of each token, while the deepest layers can focus on longer sequences. The Longformer combines dilated sliding window attention with global attention for some task-specific tokens. This means that full-self attention is computed for some hand-picked tokens across all layers so that they attend to all tokens, and all tokens can attend to them. For instance, in a classification task the $\texttt{[CLS]}$ is allowed to attend to all tokens through global attention, improving its final  encoded representation. Since global attention is only computed for few tokens, it does not impact the overall (linear) complexity of the Longformer attention. These approximations allow the Longformer to model sequences of up to 32,000 tokens, a considerable improvement over the default input size of models with quadratic attention, like BERT, which has $\tfslen = 512$. It is worth noting that computing (dilated) slided window attention in the most efficient way requires writing custom CUDA kernels. This restricts the applicability of Longformers to hardware architectures that support CUDA, excluding, for instance, Tensor Processing Units (TPUs) that would otherwise be able to support a transformer model.    


==> chapters/todo-outline.tex <==

% \chapter{Tokenization}\label{sec:tokenization}
% \input{chapters/tokenization/tokenization.tex}
% \newpage{}

% \section{Byte-Pair Encoding}\label{sec:bpe}
% \input{chapters/tokenization/bpe.tex}
% \newpage{}

% \section{Information Theory and NLP Performance}\label{sec:tokenization_information_theory}
% \input{chapters/tokenization/information_theory.tex}

% \chapter{Sampling from a Language Model}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%% CHAPTER Curating a Corpus %%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \chapter{Curating a Corpus}

% \section{Building a Corpus}

% \section{Tokenization}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%% CHAPTER Generating Text %%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \section{Sampling from a Language Model}\label{sec:generating}
% \input{chapters/estimation_sampling/sampling}
% Since a language model gives us a distribution over strings, sampling from a language model naturally produces strings. 
% Given the autoregressive 
% One of the most popular use-cases for language models is text generation. 


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%% CHAPTER System %%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \chapter{System}

% \section{Parallelism}



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%% CHAPTER Evaluation, Analysis, and Applications %%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \chapter{Evaluation, Analysis and Applications}

% \section{Probing}

% \section{Pre-training and Fine-tuning}

% \section{Promping}

% \section{Cognitive Modeling}

% \section{Ethical Concerns}

% \section{Outlook}


==> chapters/tokenization/bpe.tex <==
Now that we understood that the best way of choosing $\alphabet$ is something between characters and words, in this section we describe a popular method to find such a \defn{tokenization}\index{tokenization} automatically from data.
For this, we turn to \defn{Byte-Pair Encoding} \index{Byte-Pair Encoding} (BPE), which was originally proposed as a compression scheme \citep{gage1994}, and later repurposed by \citet{sennrich2016} for finding $\alphabet$ for a machine translation system.

We first provide an intuitive description and illustration of this algorithm, then its formal treatment, resulting in the main theorem of this section and finally conclude with an analysis of the algorithm.

\subsection{Intuition}

Given some text $\str \in \alphabetchar^*$, we separate it into individual characters in $\alphabetchar$, which we all add to $\alphabet$, so that $\alphabetchar \subset \alphabet$.
Then we repeatedly concatenate the most frequent neighbouring strings, each time adding the result to $\alphabet$.
We stop when we reach some criteria, such as $\alphabet$ being of sufficient size.
Notice that in \Cref{tab:micro_bpe_example} we arrived, without any knowledge of morphology, at a tokenization between character and word-level.
It is easy to see that this algorithm is indeed a \defn{compression} \index{compression} algorithm where we try to minimize the number of symbols that we need to transfer, with the contraint on the total number of unique symbols.

With the final alphabet of $\alphabet = \alphabetchar \cup \{ \textit{pi, pic, pick, ed} \}$ we are able to \defn{encode} \index{encoding} all words.
For example \textit{picking} would be encoded as $\langle \textit{pick, i, n, g} \rangle$ and for \textit{armadilo} we would have to fall-back to the elements in $\alphabetchar$: $\langle \textit{a, r, m, a, d,}$ $\textit{i, l, o} \rangle$.
It is clear that the efficiency of the encoding hinges on which symbols $\alphabet$ is composed of.
If the word to be encoded contains long segments from $\alphabet$, it can be encoded efficiently.
Otherwise, we have to resort to character-level representation.
Importantly, we are able to represent all words but also remain efficient in this representation.

\begin{table}[htbp]
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lc}
            \toprule
            \bf Text                                                                                                        & \bf Addition to $\alphabet$ \\
            \midrule
            \texttt{\mergeemph{p i} c k e d \, \mergeemph{p i} c k l e d \, \mergeemph{p i} c k l e s}                      &
            $\{ p, i, c, k, e, d, l, s \}$                                                                                                                \\
            \texttt{pi \mergeemph{c k} e d \hspace{3.5mm} pi \mergeemph{c k} l e d \hspace{2.5mm} pi \mergeemph{c k} l e s} &
            $\{ pi \}$                                                                                                                                    \\
            \texttt{\mergeemph{pi ck} e d \hspace{4.1mm} \mergeemph{pi ck} l e d \hspace{4.3mm} \mergeemph{pi ck} l e s}    &
            $\{ ck \}$                                                                                                                                    \\
            \texttt{pick \mergeemph{e d} \hspace{7.0mm} pick l \mergeemph{e d} \hspace{6.2mm} pick l e s}                   &
            $\{ pick \}$                                                                                                                                  \\
            \texttt{pick ed \hspace{10.0mm} \mergeemph{pick l} ed \hspace{8.3mm} \mergeemph{pick l} e s}                    &
            $\{ ed \}$                                                                                                                                    \\
            \texttt{pick ed \hspace{10.9mm} pickl ed \hspace{12.2mm} pickl e s}                                             &
            $\{pickl\}$                                                                                                                                   \\
            \bottomrule
        \end{tabular}
    }
    \captionof{myexamplef}{Compression of the text sequence \textit{picked pickled pickles} using 5 greedy merges according to the BPE algorithm. The most frequently occurring pair of vocabulary items is highlighted and merged in the next iteration.}
    \label{tab:micro_bpe_example}
\end{table}

This algorithm is known as greedy BPE and we provide a minimal Python implementation in \Cref{code:minimal_bpe}.
For a proper mathematical description of the algorithm, we first develop the notation and formalisms.
The variable $M$ is a hyperparameter which corresponds to the number of merges that will take place.
In turn, this affects the overall vocabulary size.

% force the float to defloat otherwise it takes up the whole page
\begin{figure}[H]
    \centering
    \begin{minted}[]{python}
from collections import Counter
from typing import Union, Tuple, List

def bpe(xs: Union[str, List], M: int):
  for _ in range(M):
    pairs = Counter(zip(xs, xs[1:]))
    top_pair = pairs.most_common(1)[0][0]
    xs = merge(list(xs), top_pair)
  return xs

def merge(xs: List, pair: Tuple):
  ys = []
  while xs:
    if tuple(xs[:2]) == pair:
      ys.append(pair)
      xs = xs[2:]
    else:
      ys.append(xs.pop(0))
  return ys 

bpe("picked pickled pickles", 4)
\end{minted}
    \captionof{codef}{A minimal implementation of greedy algorithm for BPE \citep{sennrich2016} in Python 3.}
    \label{code:minimal_bpe}
\end{figure}

\subsection{Formal Treatment}

So far we used the notions of ``selecting $\alphabet$'' and ``tokenization'' interchangeably.
They are, however, not the same thing.
Our primary goal is to split $\str$ into segments given some criteria.
Commonly those are that the total number of segments is small and that the set of all occurred segments

The fundamental building block of the BPE problem is a merge, which we define formally below.
Informally, a merge is the action of creating a new symbol out of two existing ones.
Out of convention, we also refer to the resulting object as a merge.

\begin{definition}
    \label{definition:merge}
    Let $\alphabet$ be an alphabet, a finite, non-empty set.
    The set of all \defn{merges} over $\alphabetchar$ is the smallest set of pairs $\alphabetmerge$ with the following closure property:
    $\mop{\merge'}{\merge''} \in \alphabetmerge $\, for $\merge', \merge'' \in \alphabettree = \alphabet\cup \alphabetmerge$.
    Note that an element $\mergetree \in \alphabettree$ can be seen as a bracketing or an ordered full binary tree over a string $\str \in \Sigma^*$.
    We denote the elements of $\alphabetmerge$ as $\merge=\mop{\merge'}{\merge''}$.
    A \defn{merge sequence} is an ordered set of merges, which we denote $\merges = \langle \merge_1, \ldots, \merge_N \rangle \in \alphabetmerge^*$.
\end{definition}

Consequently, the repeated application of different merges leads to the notion of a merge sequence and its application, which connects the set $\alphabet$ and tokenization of text.

\begin{definition}\label{def:valid}
    We define a merge sequence $\merges = \langle \merge_1, \ldots, \merge_N \rangle \in \alphabetmerge^*$ to be \defn{valid} if, for every $ \merge_n $, it holds that $ \merge_n = \mop{\merge_n^1}{\merge_n^2}$, where for $i\in\{1,2\}$ either $\merge_n^i = \merge_k$ with $k<n$, or $\merge_k^i \in \alphabetchar$. We denote the set of valid merge sequences $\validmerges$.
\end{definition}

We denote the \defn{application} of a merge sequence $\merges = \langle \merge_1, \ldots, \merge_N\rangle$ to a string $\str \in \alphabet^*$ as $\encmerge_{\merges}(\str)$.
To apply a single merge $\merge_i$, we first consider $\singleencmerge_{\merge_i}(\treesmerge_{\str})$, where $\treesmerge_{\str}$ is the canonical representation of $\str$ in $\alphabettree^*$.
Then, we replace all $\treemerge_{\str}^{k}, \treemerge_{\str}^{k+1}$ in $\treesmerge_{\str}$ such that $(\treemerge_{\str}^{k}, \treemerge_{\str}^{k+1})=\merge_i$ by $\merge_i$ itself, in a left-to-right fashion.
We thus obtain a new $\treesmerge_{\str}' \in \alphabettree^*$, to which a new single merge can be applied. The application of a merge sequence over a string $\str $ can then be viewed as this iteration of $\singleencmerge$ on $\treesmerge_{\str}$ for the successive $\merge_i$ in $\merges$. As a result, we obtain $\treesmerge_{\str}^{\dagger} \in \alphabettree^*$ a non-overlapping ordered forest, i.e., partial bracketing of $\str$.
We provide an example in \Cref{fig:merge_tree_example}.
The quantity $|\encmerge_{\merges}(\str)|$ is the number of elements in the sequence, which also corresponds to the number of trees in $\treesmerge_{\str}^{\dagger}$.
Note that the application of the merge sequence is deterministic.

\begin{figure}
    \centering
    % There's surely a better way of doing this than with absolute coords -vilem
    \begin{tikzpicture}[
            scale=0.75,
            char/.style={
                    text height={height("a")+0pt},
                    text width={width("a")+0pt},
                    inner sep=1mm,
                    align=center,
                    font=\fontsize{11}{0}\selectfont\itshape,
                },
            subword/.style={
                    align=center,
                    font=\fontsize{11}{0}\selectfont,
                },
            merge/.style={
                    draw,
                    circle,
                    align=center,
                    line width=0.35mm,
                    inner sep=0.7mm,
                },
            connector/.style={
                    line width=0.4mm
                }
        ]
        \node[char] at (0, 0) (r0c0) {a};
        \node[char] at (1, 0) (r0c1) {b};
        \node[char] at (2, 0) (r0c2) {a};
        \node[char] at (3, 0) (r0c3) {a};
        \node[char] at (4, 0) (r0c4) {b};
        \node[char] at (5, 0) (r0c5) {a};
        \node[char] at (6, 0) (r0c6) {c};
        \node[char] at (7, 0) (r0c7) {b};
        \node[char] at (8, 0) (r0c8) {c};
        \node[char] at (9, 0) (r0c9) {b};

        \node[merge] at (0.5, 1.1) (r1c0) {$\merge_1$};
        \node[merge] at (3.5, 1.1) (r1c1) {$\merge_1$};
        \node[merge] at (6.5, 1.1) (r1c2) {$\merge_2$};
        \node[merge] at (8.5, 1.1) (r1c3) {$\merge_2$};
        \node[merge] at (1.25, 2.2) (r2c0) {$\merge_3$};
        \node[merge] at (4.25, 2.2) (r2c1) {$\merge_3$};
        \node[merge] at (5.375, 3.3) (r3c0) {$\merge_4$};

        \draw[connector] (r1c0) -- (r0c0);
        \draw[connector] (r1c0) -- (r0c1);
        \draw[connector] (r2c0) -- (r1c0);
        \draw[connector] (r2c0) -- (r0c2);

        \draw[connector] (r1c1) -- (r0c3);
        \draw[connector] (r1c1) -- (r0c4);
        \draw[connector] (r1c2) -- (r0c6);
        \draw[connector] (r1c2) -- (r0c7);
        \draw[connector] (r2c1) -- (r1c1);
        \draw[connector] (r2c1) -- (r0c5);
        \draw[connector] (r3c0) -- (r2c1);
        \draw[connector] (r3c0) -- (r1c2);

        \draw[connector] (r1c3) -- (r0c8);
        \draw[connector] (r1c3) -- (r0c9);

        \node[subword] at (1, -0.7) {$\mopt{\mopt{a}{b}}{a}$};
        \node[subword] at (5, -0.7) {$\mop{\mopt{\mopt{a}{b}}{a}}{\mopt{c}{b}}$};
        \node[subword] at (8.5, -0.7) {$\mopt{c}{b}$};
    \end{tikzpicture}

    % \includegraphics[width=0.9\linewidth]{img/merge_tree_example.pdf}
    \vspace{-2mm}
    \caption{Application of the merge sequence $\merges = \langle \mop{a}{b},$ $\mop{c}{b}, \mop{\mop{a}{b}}{a},$ $\mop{\mop{\mop{a}{b}}{a}}{\mop{c}{b}}\rangle$ on the string $\str = abaabacbcb$. The result can be represented as an ordered forest. Each tree is associated with a subword in the text: $aba$, $abacb$, and $cb$.}
    \label{fig:merge_tree_example}
\end{figure}


\begin{definition}
    \label{def:yield}
    The \defn{yield} of $\treemerge \in \alphabettree$, denoted as $\yieldmerge(\treemerge)$, is defined recursively as follows:
    \begin{equation}
        \hspace{-1mm}\yieldmerge(\treemerge) =
        \begin{cases}
            \treemerge                                         & \hspace{-3mm} \textbf{if } \treemerge \in \alphabetchar               \\
            \yieldmerge(\treemerge') \yieldmerge(\treemerge'') & \hspace{-3mm} \textbf{if } \treemerge=\mop{\treemerge'}{\treemerge''}
        \end{cases}
    \end{equation}
\end{definition}

As an example, $\yield(\mop{\mop{a}{a}}{\mop{\mop{c}{b}}{c}})$ is $aacbc$.
It is easy to see that the yields of merges are the \defn{subwords} \index{subword} used in downstream applications.
Coming back to the example in \Cref{tab:micro_bpe_example}, the sequence would be represented as $\langle$ pick, ed, \,, pickl, ed, \, pickl, e, s $\rangle$ even though the corresponding merge tree is more complex (e.g. $\mop{\mop{\mop{p}{i}}{c}}{k}$ for the first token).

\section{BPE Training \& Analysis}

Now we know that the BPE algorithm jointly finds a merge sequence $\merges$ and at the same time tokenize string $\str$.
Note that even though it does two things at once, the merge sequence $\merges$ can also be applied on another string, $\str'$, which was not seen during the training.
This corresponds to our knowledge of modern applications, where a system is deployed, expects input to be preprocessed (tokenized) consistently and accepts queries which are different from those during training.
We do not describe in detail the algorithm by which unseen words are merged, though there are several commonly used.
The simplest one applies all possible merge operations from $\merges$ onto the word.

Because there are multiple ways of obtaining a merge sequence $\merges$ and BPE is only one of such algorithm, it is important to be able to measure the goodness of the merge sequence with respect to a specific string $\str$.
Recall, that we referred to BPE as originally a compression algorithm and so we may consider the quantity of how much space is saved after applying the merge sequence.

\begin{definition}
    \label{defn:compression}
    Let $\str \in \alphabetchar^*$ be a string.
    We define the \defn{compression utility} of a valid merge sequence $\merges$ applied to $\str$ as the following function:
    \begin{equation}
        \computil_{\str}(\merges) = |\str| - |\encmerge_{\merges}(\str)|
    \end{equation}
    Note that $\computil_{\str}(\langle \rangle) = 0$, for any merge sequence $\merges$, $\computil_{\str}(\merges) \geq 0$.
    Then, for any merge sequence $\merges' = \langle \merge_1, \ldots, \merge_{|\str|-1} \rangle$ of length $|\str|-1$  where every merge produces replacements, we have $\computil_{\str}(\merges') = |\str|-1$.
\end{definition}

% \subsection{Algorithm Analysis}

With the previous definition we can more formally present the algorithm.
It is the more straightforward implementation, though there exist algorithms which solve the exactly same problem but faster.

\begin{algorithm}[htbp]
    % {\fontsize{11}{12}\selectfont
    \begin{algorithmic}[1]
        \State $\merges \gets \langle \rangle$
        \State $\treesmerge \gets \treesmerge{\str}$
        \For{$i \text{ in } \{0,\ldots,M\}$}
        \State
        $\merge \gets \argmax_{(\treemerge', \treemerge'') \in \text{set}(\treesmerge)^2}$
        $\Call{PairFreq}{\treesmerge, (\treemerge',\treemerge'')}$
        \label{algo:iterative_greedy_bpe_slow_line_pairs}
        \State
        $\treesmerge \gets \Call{SingleApply}{\merge,\treesmerge}$
        \label{algo:iterative_greedy_bpe_slow_line_merge}
        \State $\merges \gets \merges \circ \langle \merge \rangle$
        \EndFor
        \State \Return $\merges, \treesmerge$
    \end{algorithmic}
    % }
    \caption{%
        Iterative Greedy BPE.\newline
        \textbf{Inputs}: sequence $\str$, merge count $M$\newline
        \textbf{Output}: merge sequence $\merges$, tokenized sequence $\treesmerge$
    }
    \label{algo:iterative_greedy_bpe_slow}
\end{algorithm}


In words, the greedy algorithm proceeds as follows:
For each of the $M$ iterations, the algorithm chooses the next merge that is both valid and (locally) minimizes the objective in \cref{eq:optimization-objective}.
We give pseudocode in \Cref{algo:iterative_greedy_bpe_slow}.
In practice, as shown in \Cref{code:minimal_bpe}, this is done by choosing the merge that occurs most frequently.
% (\Cref{def:compression_gain_utility})
The main loop occurs $M$ times.
Assuming constant-time comparison of strings, finding the maximum pair count over the whole string is $\bigO{N}$, which is the same as applying one merge.
Overall, this yields to runtime complexity of $\bigO{MN}$.

% A large amount of time in the slow BPE implementation, presented by \citet{sennrich2016} and shown in \Cref{algo:iterative_greedy_bpe_slow}, is spent on
% \begin{enumerate*}
% \item recalculating the frequencies of pairs (\Cref{algo:iterative_greedy_bpe_slow}, line \ref{algo:iterative_greedy_bpe_slow_line_pairs}) which are not affected by the most recent merge, and
% \item scanning the whole string to apply a single merge (\Cref{algo:iterative_greedy_bpe_slow}, line \ref{algo:iterative_greedy_bpe_slow_line_merge}).
% \end{enumerate*}
% To make this explicit, consider the following example.\looseness=-1
% \begin{myexample}
% Consider $\str = abba (cddc)^n$ and merge $\mop{a}{b}$ for $n \geq 1$.
% % \ryan{We need to say whether the naturals have 0. Otherwise, this is underspecified.}
% We can only apply the merge at the beginning of the string, which results in the forest $\mop{a}{b}ba (cddc)^n$.
% However, \Cref{algo:iterative_greedy_bpe_faster} still scans the entirety of the sequence to recalculate the pair frequencies of $\mop{c}{d}, \mop{d}{c}$ and $\mop{c}{c}$.
% This additional work is unnecessary.\looseness=-1
% \end{myexample}

\section{Optimality Analysis}

% We need to give some basic theory that byte-pair encoding is at best locally optimal and discuss its runtime

The way we described the BPE algorithm and for which we provided the pseudocode in \Cref{code:minimal_bpe}, is its \textit{greedy} variant.
This is because we are not searching through the whole space of $\{\merges \in \validmerges | \merges| \leq M\}$ but instead build it iteratively and greedily in $M$ steps.
We can also now state what combinatorical objective is the BPE algorithm optimizing, which happens to be finding $\merges$ such that they maximize $\computil_{\str}(\merges)$.
\begin{equation}\label{eq:optimization-objective}
    \mergesopt = \argmax_{\substack{\merges \in \validmerges, \\ |\merges| \leq M}} \computil_{\str}(\merges)
\end{equation}

We first define several functions that we will use to prove a specific property of $\computil$, submodularity, which is needed to show that the greedy algorithm is not arbitrarily bad.
Specifically, given optimal merge sequence $\mergesopt$ and greedy merge sequence $\mergesgreedy$, we wish to show that
\begin{equation}
    \frac{\computil_{\str}(\mergesgreedy)}{\computil_{\str}(\mergesopt)} \geq 1 - \sfrac{1}{e}
\end{equation}

We start by proving some useful facts about the compression utility function $\computil_{\str}$.
Specifically, we first show that $\computil_{\str}$ is a specific type of monotone non-decreasing submodular sequence function, which we make precise in the following definitions.
\begin{definition}\label{def:monotone}
    A real-valued function $f$ over valid merge sequences is \defn{monotone non-decreasing} if, for all $\merges \in \validmerges$ and for all $n \in \N$, it holds that $f(\merges_{< n}) \geq f(\merges_{<n-1})$.
\end{definition}

The following definition is introduced only for stylistic convenience.

\begin{definition}
    \label{def:compression_gain_utility}
    The \defn{compression gain} of $\merges'$ with respect to another sequence $\merges$, denoted as $\computil_{\str}(\merges' \mid \merges)$, is defined as $\computil_{\str}(\merges  \merges') - \computil_{\str}(\merges)$.
    Similarly, the compression gain of a single merge $\merge$ with respect to a sequence $\merges$, denoted as $\computil_{\str}(\merge \mid \merges)$, is defined as $\computil_{\str}(\merges  \merge) - \computil_{\str}(\merges)$.\footnote{$\merges\merges'$ is a sequence concatenation.}
\end{definition}

\begin{proposition}{}{}
    Let $\computil_{\str}$ be the compression utility function.
    Then, for a fixed $\str \in \alphabet^*$, $\computil_{\str}(\cdot)$ is monotone (\Cref{def:monotone}).
\end{proposition}

\begin{proof}
    For all $n \in \N$, we have that $\computil{\str}(\merges_{<n}) =\allowbreak \computil_{\str}(\merges_{<n-1}) + \underbrace{\computil_{\str}(\merge_n \mid \merges_{<n-1})}_{\geq 0}$.
    It follows that $\computil_{\str}(\cdot)$ is monotone non-decreasing.
\end{proof}

Next, we turn to a definition of sequence submodularity.
In contrast to the usual definitions, we add the additional constraint that merge-sequence function must take a \emph{valid} merge sequence as an argument.
\begin{definition}\label{def:submodular} \index{sequence submodularity}
    A real-valued function $f$ over valid merge sequences is \defn{submodular} if, for all  $\merges, \merges' \in \validmerges$ such that $\merges' \preccurlyeq \merges$,\footnote{I.e., we have that $\merges'$ is a prefix of $\merges$.} and for all $\nu \in \alphabetmerge$ such that both $\merges' \nu$ and $\merges \nu$ are valid, we have
    \begin{equation}
        \label{eq:function_submodularity}
        f(\nu \mid \merges') \geq f(\nu \mid \merges).
    \end{equation}
\end{definition}

\begin{proposition}{}{}
    Let $\computil_{\str}$ be the compression utility function.
    Then, for a fixed $\str \in \alphabet^*$, $\computil_{\str}(\cdot)$ is submodular (\Cref{def:submodular}) when the domain is restricted to the set of valid merges $\validmerges$.
\end{proposition}

\begin{proof}
    Let $\merges, \merges' \in \validmerges$ be two valid merge sequences such that $\merges \preccurlyeq \merges'$.
    Combinatorially, $\computil_{\str}(\merges\nu) - \computil_{\str}(\merges)$ is the number of new nodes added to the forest induced by applying $\nu$ to $\str$ after $\merges$ was already applied to $\str$.
    Likewise, $\computil_{\str}(\merges'\nu) - \computil_{\str}(\merges')$ is the number of new nodes added to the forest induced by applying $\nu$ to $\str$ after $\merges'$ was already applied to $\str$.
    However, because $\merges$ is a prefix of $\merges'$, the number of nodes created by applying $\nu$ after $\merges'$ is applied must be less than or equal to the number created after $\merges$ is applied.
    Because both $\merges'\nu$ and $\merges\nu \in \validmerges$, this shows $\computil_{\str}(\merges'\nu) - \computil_{\str}(\merges') \leq \computil_{\str}(\merges\nu) - \computil_{\str}(\merges)$, which proves submodularity.
\end{proof}


Another way of understanding the submodularity of $\computil_{\str}(\cdot)$ is in terms of the compression gain function.
We can simply write that
\begin{equation}
    \computil_{\str}(\nu \mid \merges') \geq \computil_{\str}(\nu \mid \merges) \qquad \text{for} \qquad \merges' \preccurlyeq \merges
\end{equation}

\begin{myexamplef}
    Consider $\alphabetchar = \{a, b, c, d, e\}$, the string $\str=aabcde$, and the valid merge sequences $\merges' = \langle \mop{a}{a} \rangle$ and $\merges = \langle \mop{a}{a}, \mop{c}{d} \rangle$.
    Note that $\merges' \preccurlyeq \merges$.
    These merge sequences have compressions $\computil_{\str}(\merges') = 6 - 5 = 1$ and $\computil_{\str}(\merges) = 6 - 4 = 2$, respectively.
    Next, consider the merge sequence $\vnu = \langle \mop{b}{\mop{c}{d}}, \mop{\mop{b}{\mop{c}{d}}}{e}\rangle$.
    Now, the tables have turned, and $\computil_{\str}(\merges' \vnu) = 6 - 5 = 1$ and $\computil_{\str}(\merges \vnu) = 6 - 2 = 4$.
    So, we have $\computil_{\str}(\merges')
        \leq \computil_{\str}(\merges)$, but
    $\computil_{\str}(\merges' \vnu) \geq \computil_{\str}(\merges \vnu)$, which violates submodularity.
    % What went wrong?
    The problem is that $\merges \vnu$ is not a \emph{valid} merge sequence.
\end{myexamplef}


In order to prove our desired guarantee, however, it is not enough that compression utility is sequence submodular over valid merges sequences.
Luckily, we identified another property of the compression utility function that allows us to push through our result.

\begin{definition}\label{defn:subset-parital-order}
    We define the following \defn{partial order on merges}.
    For merges $\merge, \merge' \in \alphabetmerge$, we say $\merge' \subset \merge$ iff
    $\merge'$ is a submerge of $\merge$.
    The merge $\merge'$ is a \defn{submerge} of $\merge = \mop{\merge_1}{\merge_2}$ iff:
    \begin{itemize}[noitemsep,topsep=0mm]
        \item $\merge_1 = \merge'$,  or, $\merge_2 = \merge'$, or
        \item $\merge' \subset \merge_1$, or $\merge' \subset \merge_2$.
    \end{itemize}
\end{definition}

\begin{definition}\label{def:hierarchical-submodular} \index{hiearchical submodularity}
    A real-valued function over valid merge sequences is \defn{hierachically sequence submodular} if, for every valid merge sequence of the form $\merges'\nu'\merges\nu$
    where $\nu' \subset \nu$ according to the partial order given in \Cref{defn:subset-parital-order}, we have that
    \begin{equation}\label{eq:hierarchical-submodularity}
        f(\nu'\mid \merges'  ) \geq f(\nu \mid \merges'  \nu'  \merges).
        % f(\nu' \merges') - f(\merges') \geq f(\nu \merges \nu' \merges') - f(\merges \nu' \merges')
    \end{equation}
    %where $f(x\mid y) \defeq f(y\circ x) - f(y)$\ryan{This ``gain'' should be defined.}
\end{definition}
Note that hierarchical sequence submodularity is a different concept from function modularity, described in \Cref{def:submodular}.
Indeed, in the case of functions over valid merge sequences, neither submodularity nor hierarchical sequence submodularity implies the other.
To see this, note that roughly speaking, submodularity describes the difference in the value of a function when the same element is given as an argument, albeit conditioned on the presence of two different (but related) other arguments.
% \gianni{I find this sentence unclear \response{clara} I chaged it quite a bit now, but still think it could use some work}
However, if the same argument is considered in \Cref{eq:hierarchical-submodularity}, we have
\begin{equation}
    \computil_{\str}(\nu \mid \merges') \geq \computil_{\str}(\nu \mid \merges' \nu' \merges) = 0,
\end{equation}
which is a trivial bound due to the non-negativity of $\computil_{\str}(\cdot)$.
The naming is inspired by the fact we require the partial order over merges, which creates the hierarchy.

% \gianni{Remember to put the definition of submerge somewhere else}
% Lastly, we define a partial ordering over $\mergealphabet$ that induces a hierarchy over the merges.


\begin{proposition}{}{hierarchical-submodular}
    Let $\computil_{\str}$ be the compression utility function.
    Then, for a fixed $\str \in \alphabet^*$, $\computil_{\str}(\cdot)$ is hierarchically submodular (\Cref{def:submodular}) when the domain is restricted to the set of valid merges $\validmerges$.
\end{proposition}

\begin{proof}
    Let $\str \in \alphabet^*$ be a string and $\merges$, $\merges'$ be valid merge sequences.
    Furthermore, let $\nu$, $\nu'$ be merges such that $\nu' \subset \nu$ and $\merges' \nu' \merges \nu$ is itself a valid merge sequence.
    Combinatorially, $\computil_{\str}(\nu \mid \merges' \nu' \merges)$ is the number of replacements made in $\treesmerge$ by the single merge of $\nu$, after applying $\merges' \nu' \merges$.
    However, since $\nu' \subset \nu$, every new tree in $\treesmerge$ resulting from that by applying $\nu$ must have $\nu'$ as a descendant.
    Thus, $\computil_{\str}(\nu' \mid \merges' )$, which is
    the number of new nodes in the forest created by applying $\nu'$, must be at least equal to $\computil_{\str}(\nu \mid \merges' \nu' \merges)$, if not greater.
\end{proof}
\Cref{prop:hierarchical-submodular} gives us a different notion of submodularity that later allows us to prove a guarantee for BPE \emph{despite} the presence of the constraint that BPE only searches over the space of valid merge sequences.
As an illustrative example of the proposition, we return to \Cref{fig:merge_tree_example}.
In this case, $\merges' = \langle \mop{a}{b} \rangle$, $\nu' = \mop{\mop{a}{b}}{a}$, $\merges = \langle \mop{c}{b} \rangle$, $\nu = \mop{\mop{\mop{a}{b}}{a}}{\mop{c}{b}}$.
Clearly, $\nu' \subset \nu$ and $\nu'$ appears twice, while $\nu$ only once.


\begin{lemma}{}{big-proof-helper}
    Let $\merges', \merges \in \validmerges$ be valid merge sequences.
    Recall the definition of the compression gain function
    \begin{equation}
        \kappa_{\str}(\merges \mid \merges') \defeq \kappa_{\str}(\merges' \merges) - \kappa_{\str}(\merges')
    \end{equation}
    Then, there exists a merge $\nu$ in $\merges$ such that $\kappa_{\str}(\nu\mid\merges') \geq \frac{\kappa_{\str}(\merges\mid\merges')}{|\merges|}$ and $\merges'\nu$ is a valid merge sequence.
    % \gianni{I get lost with the order of the compositions. Shouldn't it be $\merges' \nu$ instead of $\merges'\nu$ here? I think this needs to be checked out throughout the paper}
\end{lemma}
\begin{proof}
    First, expand $\merges = \langle \merge_1, \ldots, \merge_T \rangle$, i.e., $\merges$ is of length $T$.
    Then, basic manipulations yield
    \begin{subequations}
        \begin{align}
            \kappa_{\str}(\merges \mid \merges') & = \kappa_{\str}(\merges' \merges) - \kappa_{\str}(\merges')                                                        & \prooftext{(definition)}      \\
                                                 & = \sum_{t=1}^T \kappa_{\str}(\merges' \merges_{<t}) - \sum_{t=0}^{T-1} \kappa_{\str}(\merges' \merges_{<t})        & \prooftext{(telescoping sum)} \\
                                                 & = \sum_{t=1}^T \Big(\kappa_{\str}(\merges' \merges_{<t}) -  \kappa_{\str}(\merges'  \merges_{<t-1}) \Big)          & \prooftext{(linearity)}       \\
                                                 & = \sum_{t=1}^T \Big(\kappa_{\str}(\merges' \merges_{<t-1} \merge_t) - \kappa_{\str}(\merges' \merges_{<t-1}) \Big) & \prooftext{(algebra)}         \\
                                                 & = \sum_{t=1}^T \kappa_{\str}(\merge_t \mid \merges' \merges_{<t-1})                                                & \prooftext{(definition)}
        \end{align}
    \end{subequations}
    Now, note that there must exist a $t' \in \{1, \ldots, T\}$ such that
    % \gianni{Isn't it $t'-1$ in the index of $\merges$ on the lhs?}
    \begin{equation}
        \kappa_{\str}(\merge_{t'} \mid \merges' \merges_{<t-1}) \geq \frac{1}{T}\sum_{t=1}^T \kappa_{\str}(\merge_t \mid \merges' \merges_{<t-1}).
    \end{equation}
    In words, this means that the maximum element of the sequence is greater or equal to the average.
    In the case of ties, choose
    the $\merge_{t'}$ with ties broken first by the partial order $\subset$ and, after that, arbitrarily if necessary.
    We consider two cases.
    \begin{itemize}
        \item \textbf{Case 1}:
              Suppose $\merge_{t'}$ is in $\merges'$.
              Then, $\frac{1}{T}\sum_{t=1}^T \kappa_{\str}(\merge_t \mid \merges' \merges_{<t-1}) = 0$, so
              $\kappa_{\str}(\merge_{t'} \mid \merges' \merges_{<t-1}) \geq \frac{1}{T}\sum_{t=1}^T \kappa_{\str}(\merge_t \mid \merges' \merges_{<t-1}) = 0$ follows from non-negativity.

        \item \textbf{Case 2}:
              Next, suppose $\merge_{t'}$ is not in $\merges'$.
              Then, suppose, by way of contradiction, that $\merges' \merge_{t'}$ was not valid.
              However, since $\merges' \merges_{<t'} \merge_{t'}$ is valid, there must exist a
              $\nu \subset \merge_{t'}$ such that $\merges' \nu$
              \emph{is} valid and $\nu$ is in $\merges$.
              We can decompose $\merges' \merges_{<t-1} \merge_t$ into $\merges' \merges_{<k} \nu \merge_{k+1 \leq t'-1}\merge_{t'}$ for some $k$.
              Now, we have
              \begin{subequations}
                  \begin{align}
                      \kappa_{\str}(\merge_{t'} \mid \merges' \merges_{<k} \nu \merges_{k+1 \leq t'-1}) & \leq \kappa_{\str}(\nu \mid \merges'\merges_{<k}) & \prooftext{(hierarchical submodularity)} \\
                                                                                                        & \leq \kappa_{\str}(\nu \mid \merges')             & \prooftext{(monotonity)}
                  \end{align}
              \end{subequations}
              But, since $\nu \subset \merge_{t'}$, we reach a contradiction because we chose $\merge_{t'}$ to be the merge that had a \emph{maximal} compression gain with ties broken by the partial order.
    \end{itemize}
    The two cases are exhaustive ($\merge_{t'} \in \merges'$ or $\merge_{t'} \notin \merges'$), proving the result.
\end{proof}


\begin{theorem}
    \label{threorem:greedy_almost_optimal}
    The greedy algorithm for BPE training is $\big(1-\sfrac{1}{e}\big)$-optimal, i.e., for every string $\str \in \alphabet^*$,
    \begin{equation}
        \frac{\computil_{\str}(\mergesgreedy)}{\computil_{\str}(\mergesopt)} \geq 1 - \sfrac{1}{e}.
    \end{equation}
\end{theorem}


\begin{proof}
    Let $\str \in \alphabet^*$ be any string.
    Let $\mergesopt$ be the valid merge sequence that maximizes $\computil_{\str}(\cdot)$ subject to the cardinality constraint that $|\mergesopt| \leq V$, and let $\mergesgreedy = \langle \greedynu_1, \ldots, \greedynu_V \rangle$ be the greedy merge sequence of length $M$ produced by \Cref{algo:iterative_greedy_bpe_slow} on $\str$.
    Note that the validity of both $\mergesopt$ and $\mergesgreedy$ implies that $\mergesgreedy\mergesopt$ is also valid.
    Now, choose a merge $\optnu$ in $\mergesopt$ according to \Cref{lem:big-proof-helper}.

    Next, we argue that
    $\computil_{\str}(\greedynu_T \mid \mergesgreedy_{<T}) \geq \computil_{\str}(\optnu \mid \mergesgreedy)$.
    We consider three cases.
    \begin{itemize}
        \item \textbf{Case 1}: Suppose $\optnu$ is in $\mergesgreedy$. Then, $\computil_{\str}(\greedynu_T \mid \mergesgreedy_{<T}) \geq \computil_{\str}(\optnu \mid \mergesgreedy) = 0$ follows by non-negativity.
        \item \textbf{Case 2}: Suppose $\optnu$ is not in $\mergesgreedy$ and $\greedynu_T \subset \optnu$, then
              $\computil_{\str}(\greedynu_T \mid \mergesgreedy_{<T}) \geq \computil_{\str}(\optnu \mid \mergesgreedy_{<T}\greedynu_T) = \computil_{\str}(\optnu \mid \mergesgreedy)$ follows from hierarchical sequence submodularity (\Cref{def:hierarchical-submodular}).

        \item \textbf{Case 3}: Suppose $\optnu$ is not in $\mergesgreedy$ and $\optnu \not\subset \greedynu_T$.
              Then, $\mergesgreedy_{<T}\optnu$ is valid.
              Now,
              \begin{subequations}
                  \begin{align}
                      \computil_{\str}(\greedynu_T \mid \mergesgreedy_{<T}) & \geq \computil_{\str}(\optnu \mid \mergesgreedy_{<T}) & \prooftext{(greedy)}        \\
                                                                            & \geq \computil_{\str}(\optnu \mid \mergesgreedy)      & \prooftext{(submodularity)}
                  \end{align}
              \end{subequations}


    \end{itemize}
    Thus, we have
    \begin{subequations}
        \begin{align}
            \computil_{\str}(\greedynu_T \mid \mergesgreedy_{<T}) & \geq \computil_{\str}(\optnu \mid \mergesgreedy)                                                       & \prooftext{(see above)}                   \\
                                                                  & \geq \frac{1}{V} \computil_{\str}(\mergesopt \mid \mergesgreedy)                                       & \prooftext{(\Cref{lem:big-proof-helper})} \\
                                                                  & = \frac{1}{V} \Big( \computil_{\str}(\mergesgreedy \mergesopt) - \computil_{\str}(\mergesgreedy) \Big) & \prooftext{(definition)}                  \\
                                                                  & \geq \frac{1}{V} \Big( \computil_{\str}(\mergesopt) - \computil_{\str}(\mergesgreedy) \Big).           & \prooftext{(monotonity)}
        \end{align}
    \end{subequations}
    %We proceed with algebraic manipulation.
    %Let $\merge$ be chosen in a locally greedy fashion such that $\computil_{\str}(\merge\mid\merges) \geq \alpha\max_{\merge} \computil_{\str}(\merge\mid\merges)$ for $\alpha \in (0, 1]$.
    %For brevity, $\computil_{\str}(\merges) = \computil_{\str}(\merges)$.
    Now, we can expand $\computil_{\str}(\greedynu_T \mid \mergesgreedy_{<T})$ to achieve
    \begin{align}
        \computil_{\str}(\mergesgreedy_{<V} \greedynu_V) - \computil_{\str}(\mergesgreedy_{<V}) & \geq \frac{1}{V} \Big( \computil_{\str}(\mergesopt) - \computil_{\str}(\mergesgreedy_{<V}) \Big).
    \end{align}
    Next, a bit more algebra results in
    \begin{subequations}
        \begin{align}
            \label{eq:inequality_l0} \computil_{\str}(\mergesgreedy) = \computil_{\str}(\mergesgreedy_{<V}\greedynu_V) & \geq \frac{1}{V} \Big( \computil_{\str}(\mergesopt) - \computil_{\str}(\mergesgreedy_{<V}) \Big) + \computil_{\str}(\mergesgreedy_{<V})      \\
                                                                                                                       & = \frac{1}{V} \computil_{\str}(\mergesopt) - \frac{1}{V}  \computil_{\str}(\mergesgreedy_{<V}) + \computil_{\str}(\mergesgreedy_{<V})        \\
                                                                                                                       & = \frac{1}{V} \computil_{\str}(\mergesopt) + \left(1 - \frac{1}{V}\right) \computil_{\str}(\mergesgreedy_{<V}). \label{eq:inequality_l_last}
            % &= \frac{1}{V} \computil_{\str}(\mergesopt) + \left(1 - \frac{1}{V}\right) \computil_{\str}(\mergesgreedy_{<V}).
        \end{align}
    \end{subequations}
    %Note that the sequence in \Cref{eq:inequality_l0} is one longer than the one in \Cref{eq:inequality_l_last}.
    %We can apply the same inequality again to $\computil_{\str}(\merges_{\leq|\merges|})$ and $\computil_{\str}(\merges_{<|\merges|})$:
    Now, we can apply the bound in \Cref{eq:inequality_l0} to itself, which yields:
    \begin{subequations}
        \begin{align}
            \computil_{\str}(\mergesgreedy) & \geq \frac{1}{V}\computil_{\str}(\mergesopt)+ \left( 1 - \frac{1}{V}\right)\left( \frac{1}{V}\computil_{\str}(\mergesopt) + \left( 1 - \frac{1}{V}\right) \computil_{\str}(\mergesgreedy_{<V-1})\right)                         \\
                                            & \geq \frac{1}{V}\left( 1 - \frac{1}{V}\right)^0\computil_{\str}(\mergesopt)+ \frac{1}{V} \left( 1 - \frac{1}{V}\right)^1 \computil_{\str}(\mergesopt) + \left( 1 - \frac{1}{V}\right)^2 \computil_{\str}(\mergesgreedy_{<V-1}).
        \end{align}
    \end{subequations}
    Recursively applying the bound results in
    \begin{subequations}
        \begin{align}
            \computil_{\str}(\mergesgreedy) & \geq \frac{1}{V} \computil_{\str}(\mergesopt) \sum_{v=0}^{V-1} \left( 1 - \frac{1}{V}\right)^v                    \\
                                            & = \frac{1}{V} \computil_{\str}(\mergesopt) \frac{1-\left( 1 - \frac{1}{V}\right)^V}{1-\left(1-\frac{1}{V}\right)} \\
                                            & = \computil_{\str}(\mergesopt) \left(1-\left( 1 - \frac{1}{V}\right)^V\right)                                     \\
                                            & = \computil_{\str}(\mergesopt) \left(1-\left[\left( 1 - \frac{1}{V}\right)^V\right]\right).
        \end{align}
    \end{subequations}
    Substituting in the inequality $x> 0 \Rightarrow \left(1-\frac{1}{x}\right)^x \leq \frac{1}{e}$, we obtain and finally arrive at
    \begin{subequations}
        \begin{align}
                 & \computil_{\str}(\mergesgreedy) \geq \left(1 - \frac{1}{e} \right) \computil_{\str}(\mergesopt) \\
            \iff & \frac{\computil_{\str}(\mergesgreedy)}{\computil_{\str}(\mergesopt)} \geq 1 - \frac{1}{e},
        \end{align}
    \end{subequations}
    which proves the result.
\end{proof}

\section{Conclusion}

The fact that greedy BPE is approximately optimal means that, compression-wise, the tokenization can not become arbitrarily bad.
However, there are other issues in this algorithm, such as susceptibility to misspellings.
If \textit{de} $\in \alphabet$ and \textit{fenestration} $\in \alphabet$, then \textit{defenestration} is going to be tokenized as $\langle \textit{de}, \textit{fenestration} \rangle$.
However, if the text is user-generated, it can be expected to contain typos, such as \textit{defeneztration}.
If this happens, then the tokenization output may change to $\langle \textit{de}, \textit{f, e, n, e, s, t, r, a, t, i, o n} \rangle$.
Now the same word with the same semantic content and with just minor surface difference is represented differently in the model, which creates issues down the line.

Finally, Byte-Pair Encoding is only one of many tokenization algorithms.
In practice, it is used with a more efficient implementation that runs faster than $\bigO{NM}$ and with a set of heuristics, pertaining especially to letter casing.

==> chapters/tokenization/information_theory.tex <==
Only very briefly 
TODO, mention Liv-Zempel
% WordPiece[https://aclanthology.org/N19-1423.pdf ] , SentencePiece[https://aclanthology.org/D18-2012.pdf ] 
% Other encoding schemes
% Readings: https://arxiv.org/abs/1808.06226 https://arxiv.org/abs/1508.07909 https://arxiv.org/abs/2004.03720 https://aclanthology.org/2021.emnlp-main.161.pdf 



==> chapters/tokenization/tokenization.tex <==
So far we assumed that text comes neatly preprocessed as a sequence of words $\str \in \alphabet$.
However, we will shortly see that there are more optimal approaches to choosing the best $\alphabet$ that have an effect on NLP applications, which is the main topic of this chapter.
The act of finding such $\alphabet$ is one part of the act of tokenization.
We first discuss several naive, albeit intuitive and baseline, approaches for choosing $\alphabet$.
% We first discuss various facts about natural language that influence $\alphabet$, e.g., morphology and syntax. 
Then, we introduce a proper formalism for tokenization and the byte-pair encoding algorithm, an automatic procedure for inducing $\alphabet$, and give an analysis of its correctness and runtime.
Finally, we expand to other approaches and attempt to capture what makes some alphabets better than others, using tools of information theory.

\paragraph{Alphabet of words.}
We intuitively understand words as sequences of characters from $\alphabetchar$, delimited by whitespace or some other special characters.
At first, we may therefore be tempted to set $\alphabet$ to be the set of all possible words: $\alphabet = \alphabetchar^*$.
This would create an infinite set, but we can limit ourselves to the set of words in a language, e.g. for English $\alphabet = \{ \text{aardvark},$ $\text{aardwolf},$ $\text{aaron}, \ldots \} \subset \alphabetchar^*$.
However, this creates the following three problems.
First, language evolves and new words and word forms are continuously being created.
Because those words are not part of the fixed $\alphabet$, they would have to be assigned a special \texttt{UNK} (unknown) token, which would mean to lose important information.
Secondly, even a modest English corpus contains close to 1 million unique tokens.
Recall from \Cref{chapter:modeling-founds} that we are interested in repeatedly modelling the distribution over words.
Should we use 4 Bytes for representing one number for probability of a single word, would need 4 MB to just represent the probability vectors across the 1 million words.
This makes it, of course, prohibitively expensive computation-wise.
\Cref{sec:general-framework} introduced the notion of embeddings, i.e. mapping from words into some vector of numbers that encode its meaning.
If ``aardvark'' and ``aardvarks'' are modelled as different units, then their embeddings do not fully leverage the clear connection between the two words and some of them occur very sparsely or maybe not at all (i.e. ``aardvark's'').

\paragraph{Alphabet of characters.}
We may attempt to fix the first problems by operating not on the level of words, but of characters.
Then, we would have the alphabet be composed of individual characters: $\alphabet = \alphabetchar = \{\_, ., !, ?, a, b, \ldots, z,$ $A, B, \ldots, Z,$ $0, 1, \ldots\}$.
This alphabet would be finite (safe for periodic additions of new characters by the Unicode standard) and would be of much smaller size than the alphabet composed of words.
With this limited size, it would be possible to both express all possible words and to have a reasonably small vocabulary vector.
This approach would also alleviate the problem of modelling some non-standard formatting using just words, such as three consecutive spaces.
In this case, they would just be three additional symbols, not formally distinguishable from characters inside of words: $\langle o, f, \,\,, a, a, d, w, a, r, k, \,', s \rangle$.
However, this creates new issues.
Firstly, now the embedding for a single unit, such as $e$, does not have a single associated meaning.
Even though this would also happen with homonyms in the previous, word-level, approach, the number of meanings of a homonym is very low.
This is in contrast to the letter $e$ appearing in more than half of all English words.
Finally, by representing text as a sequence of characters, the input sequences become much larger.
While ``a quick brown fox jumped over the lazy dog'' contains 9 words, it has 42 characters.
This becomes an issue e.g. with attention mechanisms (\Cref{sec:transformers}), which become less effective with longer sequences.

\paragraph{Alphabet of morphemes.}
The previous issues point to the optimal $\alphabet$ being somewhere between character and word level.
A linguistically motivated approach is to use morphemes as the units in $\alphabet$.
This would reduce the size of $\alphabet$ and allow for more meaningful semantic compositionality, helping with the embedding problem.
The word ``aadwark's'' would then be represented as $\langle \text{aadwark}, \text{'s} \rangle$.
While this approach is included in the list of intuitive baselines, it is not far from state-of-the-art approaches.
The only limitation is that it either requires an existing morphological model or some unsupervised approach.
Indeed, this has been a popular approach not so long ago \cite{smit2014morfessor}. 


==> exercises/modern-lms.tex <==
\begin{Exercise}[label={exercise:rnn-time-complexity}]
    \craf{def:rnn-encoding-fn} defined the RNN encoding function of a general RNN. 
    An importnat practical aspect in language modeling is the question of how quickly the context representations $\encRNN\left(\strltplus\right)$ can be computed.
    What is the time complexity of computing $\encRNN\left(\strltplus\right)$ w.r.t. $\tstep$?
\end{Exercise}

==> figures/tikz-figures/GRU.tex <==
\newcommand{\empt}[2]{$#1_{#2}$}
\begin{tikzpicture}[
    % GLOBAL CFG
    font=\sf \scriptsize,
    >=LaTeX,
    % Styles
    cell/.style={% For the main box
        rectangle, 
        rounded corners=5mm, 
        draw,
        very thick,
        },
    operator/.style={%For operators like +  and  x
        circle,
        draw,
        inner sep=-0.5pt,
        minimum height =.2cm,
        },
    function/.style={%For functions
        ellipse,
        draw,
        inner sep=1pt
        },
    ct/.style={% For external inputs and outputs
        circle,
        draw,
        line width = .75pt,
        minimum width=1cm,
        inner sep=1pt,
        },
    gt/.style={% For internal inputs
        rectangle,
        draw,
        minimum width=4mm,
        minimum height=3mm,
        inner sep=1pt
        },
    mylabel/.style={% something new that I have learned
        font=\scriptsize\sffamily
        },
    ArrowC1/.style={% Arrows with rounded corners
        rounded corners=.25cm,
        thick,
        },
    ArrowC2/.style={% Arrows with big rounded corners
        rounded corners=.5cm,
        thick,
        },
    ]

%Start drawing the thing...    
    % Draw the cell: 
    \node [cell, minimum height =4cm, minimum width=6cm] at (0,0){} ;

    % Draw inputs named ibox#
    \node [gt, label={[mylabel]above: \hspace{-6 mm} \empt{f}{t}}] (ibox1) at (-2,-0.75) {$\sigma$};
    \node [gt] (ibox2) at (-1.5,-0.75) {$\sigma$};
    \node [gt, label={[mylabel]above:\quad\quad\quad\empt{g}{t}} ,minimum width=1cm] (ibox3) at (-0.5,-0.75) {Tanh};
    \node [gt] (ibox4) at (0.5,-0.75) {$\sigma$};

   % Draw opérators   named mux# , add# and func#
    \node [operator] (mux1) at (-2,1.5) {$\times$};
    \node [operator] (add1) at (-0.5,1.5) {+};
    \node [operator, label={[mylabel]left: \hspace{-12 mm}\empt{i}{t}}] (mux2) at (-0.5,0) {$\times$};
    \node [operator,label={[mylabel]left: \hspace{-12 mm}\empt{o}{t}} ] (mux3) at (1.5,0) {$\times$};
    \node [function] (func1) at (1.5,0.75) {Tanh};

    % Draw External inputs? named as basis c,h,x
    \node[ct, label={[mylabel]Cell}] (c) at (-4,1.5) {\empt{c}{t-1}};
    \node[ct, label={[mylabel]Hidden}] (h) at (-4,-1.5) {\empt{h}{t-1}};
    \node[ct, label={[mylabel]left:Input}] (x) at (-2.5,-3) {e'\empt{y}{t}};

    % Draw External outputs? named as basis c2,h2,x2
    \node[ct ] (c2) at (4,1.5) {\empt{c}{t}};
    \node[ct ] (h2) at (4,-1.5) {\empt{h}{t}};
    \node[ct ] (x2) at (2.5,3) {\empt{h}{t}};

% Start connecting all.
    %Intersections and displacements are used. 
    % Drawing arrows    
    % \draw [ArrowC1] (c) -- (mux1) -- (add1) -- (c2);

    % % Inputs
    % \draw [ArrowC2] (h) -| (ibox4);
    % \draw [ArrowC1] (h -| ibox2)++(-0.5,0) -| (ibox2);
    % \draw [ArrowC1] (h -| ibox3)++(-0.5,0) -| (ibox3);
    % \draw [ArrowC1] (x) -- (x |- h)-| (ibox3);

    % % Internal
    % \draw [->, ArrowC2] (ibox1) -- (mux1);
    % \draw [->, ArrowC2] (ibox2) |- (mux2);
    % \draw [->, ArrowC2] (ibox3) -- (mux2);
    % \draw [->, ArrowC2] (ibox4) |- (mux3);
    % \draw [->, ArrowC2] (mux2) -- (add1);
    % \draw [->, ArrowC1] (add1 -| func1)++(-0.5,0) -| (func1);
    % \draw [->, ArrowC2] (func1) -- (mux3);

    % %Outputs
    % \draw [-, ArrowC2] (mux3) |- (h2);
    % \draw (c2 -| x2) ++(0,-0.1) coordinate (i1);
    % \draw [-, ArrowC2] (h2 -| x2)++(-0.5,0) -| (i1);
    % \draw [-, ArrowC2] (i1)++(0,0.2) -- (x2);

\end{tikzpicture}
